Scalable CP Decomposition for Tensor Learning using GPU Tensor Cores

CP decomposition is a powerful tool for data science, especially gene analysis, deep learning, and quantum computation. However, the application of tensor decomposition is largely hindered by the exponential increment of the computational complexity and storage consumption with the size of tensors. While the data in our real world is usually presented as trillion- or even exascale-scale tensors, existing work can only support billion-scale scale tensors. In our work, we propose the Exascale-Tensor to mitigate the significant gap. Specifically, we propose a compression-based tensor decomposition framework, namely the exascale-tensor, to support exascale tensor decomposition. Then, we carefully analyze the inherent parallelism and propose a bag of strategies to improve computational efficiency. Last, we conduct experiments to decompose tensors ranging from million-scale to trillion-scale for evaluation. Compared to the baselines, the exascale-tensor supports 8,000x larger tensors and a speedup up to 6.95x. We also apply our method to two real-world applications, including gene analysis and tensor layer neural networks, of which the numeric results demonstrate the scalability and effectiveness of our method.

==> Efficient.tex <==
\section{High Performance Exascale Implemetation}


In this section, we will first give an overall optimization on GPU implementation against the above parallel analysis, including designing efficient data storage, reducing communication overhead and improving  the utilization of GPUs. Then we will carefully design and implement optimization scheme on compression and decomposition stage respectively. 

%In this section, we will first give a roughly theoretical analysis of the maximum size of the tensors our methods supported, and show an feasible scheme for supporting exascale tensors. Then we will specifically point out the bottlenecks that limit the performance. Against the above analysis, we propose some optimization methods to improve the efficiency including optimizing the data storage, reducing communication overhead, improving the utilization of GPUs and so on. 



% In the following sections, we will focus on optimize data storage, device communications, key operations on each stage to design and implement an high performance \textit{trillion-tensor} scheme on GPU. 



%We profiled both the CPU Python implementations of our trillion-tensor scheme for dense and sparse tensorss, and found that the compression stage took most of the time of the total running time for  these algorithms with the size of tensors increasing, while for relative small sizes of tensors, the factorization stage was the bottleneck to limit the efficiency of the algorithms. Thus, for large scale tensors, we can significantly improve the performance on the compression stage to accelerate the trillion-tensor scheme both for dense and sparse tensors.

%On the compression stage, the algorithm scheme both for dense and sparse tensorss exploits the Equation (\ref{compression_equation}) to compress the large scale tensor to $P$ replicas, while for sparse tensors, $P=1$. It can be rewritten as the following iterative process:
%\begin{equation}
%\label{compress equal matrix}
%    \begin{split}
%        \mathcal{Y}&=\mathcal{X}\\
%        \bm{Y}_{(1)}&=\bm{U}\bm{X}_{(1)}\\
%        \bm{Y}_{(3)}&=\bm{W}\bm{Y}_{(3)}\\
%        \bm{Y}_{(2)}&=\bm{V}\bm{Y}_{(2)},
%    \end{split}
%\end{equation}
%with updating the replica $\mathcal{Y}$ and its matricization forms along all modes after each step. This process involves intensive computations and data transfer operations including matrix multiplication, tensor matricization and matrix folding. Compared to CPU, GPU is more suitable for large scale matrix multiplication and other data-independent operations for its much greater number of relatively unexceptional processing cores. For the factorization stage both for dense and sparse tensorss, iterative computations involved solve large scale linear square problems can also be significantly accelerated benefit from the perfect CUDA library in python. So we offload these computations in our scheme from CPU to GPU and focus on designing  and implementing our high performance trillion-tensor scheme on GPU. 



 
 
 
 
 %The data is default to computation in row-major format for the build-insert functions in Python  and supplied  APIs in Numpy. Thus, we store the data in row-major format. 
  
 %There is one disadvantage using this format that some routines in the pyCUDA libraries use the column-major format. The most time consuming key operation on the compression stage  is the matrix multiplication and it utilizes the cublasDgemm routine in pyCUDA library that uses  the column-major format. But the conflict can be solved by the latent matrix transpose with no additional compution and storage overhead. 
 
 %For example of the computation of $\bm{C}=\bm{A}\bm{B}$, due to the row-major storage format, the libraries actually take $\bm{A}^{T}$ and $\bm{B}^{T}$ as operand. Thus, we can transpose both the LHS and RHS to give $\bm{C}^{T}=\bm{B}^{T}\bm{A}^{T}$. Notice that there is no explicit matrix transpose, due to the $1D$ linear storage, $\bm{C}^{T}$ in column-major format is actually $\bm{C}$ in row-major format. The other operations depend on column-major used in CUDA libraries  consume less, the transformation of data storage format will not bring much consumption. Comprehensive consideration makes us adopt the row-major format.







\subsection{Optimization Compression Stage}

The compression process of tensor $\mathcal{X}$ for an replica $\mathcal{Y}_{p}$ for line 2 in Alg. \ref{alg:Twice compression Framwork} and Eq. \ref{compression_equation}  can be rewritten as following according to Eq. \ref{compression_equation},
\begin{equation}
    \label{compress equal matrix}\begin{split}
    \bm{y}_{p}&=\textbf{Vec}(\mathcal{Y}_{p})\\
    &=({\bm{U}_{p}}\otimes{\bm{V}_{p}}\otimes{\bm{W}_{p}})(\bm{A}\odot\bm{B}\odot\bm{C})\\
    &=((\bm{U}_{p}\bm{A})\odot(\bm{V}_{p}\bm{B})\odot(\bm{W}_{p}\bm{C})),
\end{split}
\end{equation}
where $\bm{U}_{p}, \bm{V}_{p}$ and $\bm{W}_{p}$ are the compression matrices to compress $\mathcal{X}$ to $\mathcal{Y}_{p}$, and $\bm{A}, \bm{B}$ and $\bm{C}$ are the latent decomposition factors of $\mathcal{X}$. i.e., $\textbf{Vec}(\mathcal{X})=(\bm{A}\odot\bm{B}\odot\bm{C})\bm{1}$.  Thus, the major computations involves three times of  matrix multiplications for every block on the computation stage. In the following sub-subsections, we mainly focus optimize the matrix multiplications on GPUs to accelerate the compression stage. 

\subsubsection{Efficient Compression Using Sparse Projection}

For the computation step in line 2 of Alg. \ref{alg:Twice compression Framwork}, we use the  random normal initialized matrix to compress the large scale tensor into small replicas. For each time of compression for one block, there exist $3$ times matrix multiplications shown in Eq.(\ref{compress equal matrix}), i.e., each time of matrix  multiplication corresponding to the compression for each dimension. Considering a tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$ and the compression replica $\mathcal{Y} \in \mathbb{R}^{L \times M \times N}$ where $I=J=K=500$ and $L=M=N=200$, take the first compression step  as example, we have the following equation,
\begin{equation}
    \bm{Y}_{(1)}=\bm{U}\bm{X}_{(1)},
\end{equation}
where $\bm{Y}_{(1)} \in \mathbb{R}^{L \times JK}$ and $\bm{X}_{(1)} \in \mathbb{R}^{I \times JK}$ are the matricization form in the I-mode respectively, and $\bm{U} \in \mathbb{R}^{L \times I}$ is the random normal compression matrix.  By multiplying  $\mathcal{X}$ with $\bm{U}$, the size of I mode is reduced. Suppose $\mathcal{X}$ are not sparse, there exist $LI^{3}=25,000,000,000$ times  of floating point multiplication computations which is massive and heavy. 

Here, we propose to use sparse projection to reduce the massive computations of floating points. Accoring the previous research \cite{verySparseProjection}, replacing non-sparse random normal distribution with sparse random normal distribution still enjoys some constant properties in the sense of statics, like the inner product and distance. Thus, we propose to offload the non sparse random projection to the sparse projection.

Correspondingly, instead of generating normal compression matrix, we construct the sparse  projection matrix  $\bm{U} \in \mathbb{R}^{L \times I}$, where $L \ll I$, containing entries
\begin{equation}
    \bm{U}(l,i)=
    \begin{cases}
\sqrt{s}, &\text{with prob. $\frac{1}{2s}$},\\
0, &\text{with prob. $1-\frac{1}{s}$},\\
-\sqrt{s}, &\text{with prob. $\frac{1}{2s}$},\\
\end{cases}
\end{equation}
where $s=\frac{I}{L}$, i.e., the compression ratio along the I-mode. The entries within each row are mutual-independent while the entries across different rows are fully independent. Each row will contains $s$ nonzero elements in expectation with saving $(1-\frac{1}{s}) \times 100\%$  floating point computations. As previous research reported, the properties of statistic are preserved with $s$ maximum up to $\frac{I}{\log I}$. Taking the compression of the above tensor $\mathcal{Y} \in \mathbb{R}^{500 \times 500 \times 500}$ for example, sparse projection will save $60\%$ floating point computations. 

\subsubsection{Mixed  Precision Acceleration using Tensor Core}


Tensor cores are programmable matrix-multiply-and-accumulate units that can deliver up to 125 Tensor TFLOPS for computations. It provides a significant acceleration for the operation $\bm{D}=\bm{A}\bm{B}+\bm{C}$, where $\bm{A},\bm{B}$ and  $\bm{C}$ are FP16 matrices while the accumulation matrices $\bm{C}$ and $\bm{D}$ are FP32 matrices. Thus, we fully make use of the properties of Tensor cores to accelerate the compression stage. 

We convert $\bm{U}_{p}$, $\bm{V}_{p}$, $\bm{W}_{p}$ and tensor block $\mathcal{B}_{n}$ read in memory from FP32 to FP16, and the accumulated replica $\mathcal{Y}_{p}$ to FP32 to perform mixed precision acceleration using tensor cores.

However, there is a high rounding error for the precision conversion of  which cause  cumulative error for the accumulation of the replicas. Here, we propose to factorize FP32 format data to FP16 format data and    its residual error from conversion. Here is an example shown in  Fig. \ref{fig:precision conversion}.  A FP32 format data $x_{32}$ is first converted to FP 16 format data $x_{16}$ with residual error $e_{16}$. To avoid numerical underflow for $e_{16}$, an advanced computation is executed with scaling of exponent term to obtain $\hat{x}_{16}$. $x_{16}$ and its corresponding residual error $\hat{x}_{16}$  participate in the following  computations. 

We make a preliminary experiment for matrix-multiply-and-accumulate operation $\bm{D}=\bm{A}\bm{B}+\bm{C}$, where $\bm{D} \in \mathbb{R}^{M \times N}, \bm{A} \in \mathbb{R}^{M \times K}, \bm{B} \in \mathbb{R}^{K \times N}, \bm{C} \in \mathbb{R}^{M \times N}$, using mixed precision methods and the results are shown in Fig. \ref{fig:precision conversion time } and Fig. \ref{fig:precision conversion error}. We denote \textit{FF} as float-float computation, \textit{HF} as half-float computation with no modification  and \textit{HFR} as half-float computation with modification using residual error. The MSE is the mean squared error of \textit{HF} or \textit{HFR} respect to \textit{FF}. It can be shown that compared with \textit{HF}, \textit{HFR} enjoys a significant improvement for computation precision with a relative small lost for speed.




The compression process can be factorize as following, 
\begin{equation}
    \label{residual error compression}
    \begin{split}
    \bm{y}_{p}=&({(\bm{U}_{p}}+\hat{\bm{U}}_{p})\otimes{(\bm{V}_{p}+\hat{\bm{V}}_{p})}\otimes{(\bm{W}_{p}+\hat{\bm{W}}_{p})})\textbf{Vec}(\mathcal{X}+\hat{\mathcal{X}})\\
    \approx &(\bm{U}\otimes\bm{V}\otimes\bm{W})\textbf{Vec}(\mathcal{X})+(\hat{\bm{U}}\otimes\bm{V}\otimes\bm{W})\textbf{Vec}(\mathcal{X})+\\
    &(\bm{U}\otimes\hat{\bm{V}}\otimes\bm{W})\textbf{Vec}(\mathcal{X})+(\bm{U}\otimes\bm{V}\otimes\hat{\bm{W}})\textbf{Vec}(\mathcal{X})+\\
    &(\bm{U}\otimes\bm{V}\otimes\bm{W})\textbf{Vec}(\hat{\mathcal{X}}),
\end{split}
\end{equation}
where $\bm{U}_{p},\bm{V}_{p},\bm{W}_{p},\mathcal{X}$ are stored in FP16 format, $\hat{\bm{U}}_{p},\hat{\bm{V}}_{p},\hat{\bm{W}}_{p},\hat{\mathcal{X}}$ are the residual error for the precision  conversion from FP32 to FP16 and we only consider the computations with first-order residual error and ignore the computations for the high-order residual error.

%where $\mathcal{\hat{X}}$ is the FP16 format and $\mathcal{\hat{X}}_{e}$ is the rounding error for conversion, i.e., $\mathcal{\hat{X}}_{e}=\mathcal{X}-\mathcal{\hat{X}}$. Then, we respectively calculate the compression replicas with $\mathcal{\hat{X}}$ and $\mathcal{\hat{X}}_{e}$ and merge to the same replica. 
 
%\begin{equation}
%    \label{compress equal matrix}\begin{split}
%    \bm{y}_{p}&=\textbf{Vec}(\mathcal{Y}_{p})\\
%    &=({\bm{U}_{p}}\otimes{\bm{V}_{p}}\otimes{\bm{W}_{p}})(\textbf{Vec}(\mathcal{X}))\\
%    &=((\bm{U}_{p}\bm{A})\odot(\bm{V}_{p}\bm{B})\odot(\bm{W}_{p}\bm{C})),
%\end{split}
%\end{equation}
 
%There is a high gap between the speed for processing floating points with single precision and the double precision for GPUs. Taking TITAN RTX as example, the theoretical performance  for floating point computation with double precision (FP64) is $509.8$ GFLOPS while that with single precision (FP32) is only up to $16.31$ TFLOPS which is slower maximum up to $31.34 \times$ . Despite of the high performance for single precision, the storage and computation with double precision enjoy a more stable and accurate result. Thus, We exploit mixed precision strategy to made a trade-off between precision and speed. 

%We convert $\bm{U}_{p}$, $\bm{V}_{p}$, $\bm{W}_{p}$ and tensor block $\mathcal{B}_{n}$ to single precision format before compressing the tensor block because compression is the time bottleneck of this stage. Once we get the replica $\mathcal{Y}_{p}^{n}$ after compression, we convert it from single precision to double precision when adding it to $\mathcal{Y}_{p}$, for addition is not time consuming at this stage, to avoid further loss of accuracy. In this way, we get about  10x speedup at compression stage while the loss is still in acceptable range. 




%For the baseline, the scheme compress each mode of tensor by Gaussian random matrices which contains massive floating point  computations. According  to some researches in analysis of big data, the Gaussian random projection can be replaced by sparse projection with a proper scale ratio, which is maximum up to $\log D$ where $D$ is the dimension of the initial data, and still enjoy a tolerant accuracy in the sense of statistics. Thus we propose to generate the  mode  compression matrices drawn from a given distribution $\{-1,0,1\}$ with a given probability $\{\frac{1}{2s},1-\frac{1}{s},\frac{1}{2s}\}$, where the compression ration is maximum up to $\frac{D}{\log D}$.

% A respective high compression ratio guarantees a sufficient sparsity in the compression mode matrices. Thus we organize the sparse compression mode matrices in CSR format and utilize the sparse matrix to matrix multiplication routine 
% in cuSparse library to reduce the massive time consuming floating point computations.





\subsubsection{Improving the  GPU Utilization}

 In regular GPU implementation, the matrix multiplications  for all blocks and all replicas are computed one by one on GPU.  However, the preliminary experiment result showed that the vanilla program did not fully utilize the resources of of GPUs.

We improve the utilization of GPUs by exploiting gemmBatched routine in cuBLAS libraries to run batch matrix multiplications in parallel on GPU. Due to the independence of all  compression replicas from one same block, we organize and compute the multiple matrix multiplications in  batches, accumulate and obtain the compression replicas in parallel. The batched scheme is illustrated in Fig. \ref{batched-schemes}.  The block tensor $\mathcal{B}_{n}$ is read from memory and respectively compressed by the batch organized ${\{\bm{U}^{n}_{p}\}}_{p=1}^{P}$, ${\{\bm{V}^{n}_{p}\}}_{p=1}^{P}$ and ${\{\bm{W}^{n}_{p}\}}_{p=1}^{P}$ to obtain the sub-relicas ${\{\mathcal{Y}^{n}_{p}\}}_{p=1}^{P}$ which will be accumulated to  ${\{\mathcal{Y}_{p}\}}_{p=1}^{P}$, where  ${\{\bm{U}^{n}_{p}\}}_{p=1}^{P}$, ${\{\bm{V}^{n}_{p}\}}_{p=1}^{P}$ and ${\{\bm{W}^{n}_{p}\}}_{p=1}^{P}$ are the components for compressing $\mathcal{B}_{n}$. 

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.20]{Figures/gemmbathced.png}
    \caption{Illustration of the batched matrix multiplication on compression stage. The  $\bm{U}^{n}_{p}, \bm{V}^{n}_{p}$ and $\bm{W}^{n}_{p}$ are organized in batches and parallely compress the block $\mathcal{B}_{n}$ to obtain $\mathcal{Y}^{n}_{p}$, $p=1,2,..., P$. }
    \label{batched-schemes}
\end{figure}


\subsection{Optimization Factorization Stage}
Our \textit{trillion-tensor} scheme mainly differs on the factorization stage between the dense and sparse conditions. For the dense condition, we permute all the factorization mode matrices of the compression replicas to a common scaling and permutations, solve a master linear square problem and obtain the the mode matrices after recovering the scaling and permutations. While for sparse condition, after factorizing the only replica into the mode matrices, we directly exploit the latent sparsity to solve the sparsity or error constraint  linear  problem using OMP-Cholesky algorithm. 


Factorization stage mainly consists of CP decomposition and solving linear square problems for factorization matrices of mode matrices. CP decomposition plays an important role in factorization stage.   Error constraint optimization from line $2$ to $13$ comprises of lots of times of solving least square problem. Thus, there remains a challenge that how to efficiently solve the linear square problems on the factorization stage. Here, we carefully design and implement the efficient strategy according to the facing situations.









%\section{Sparse Tensor and Multi-GPU Implementations}
 
% Multi-GPU 是技巧
 
%In this section, we will introduce our strategies for sparse tensor decomposition in \textit{exascale-tensor} scheme and show the implementations of multi GPUs.

%\subsection{Sparse Exascale-Tensor Decomposition}

%\begin{algorithm}[t] 
%\caption{Our Trillion-Tensor Scheme for Sparse Tensors} 
%\label{alg:Framworkforsparse} 
%\begin{algorithmic}[1] %这个1 表示每一行都显示数字
%\REQUIRE ~~\\ %算法的输入参数：Input
%tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$ with rank R; size of compression replicas, %$L, M, N$; 
%\ENSURE %算法的输出：Output
%mode matrices $(\bm{A}, \bm{B}, \bm{C})$;\\
%\STATE Randomly generate matrices $\bm{U}\in\mathbb{R}^{L \times I},\bm{V}\in\mathbb{R}^{M \times %J},\bm{W}\in\mathbb{R}^{N \times K}$,
%\label{ code:fram:compression }%对此行的标记，方便在文中引用算法的某个步骤
%%\FOR{$p=1$ to $P$}
%\STATE $\mathcal{Y} \gets$ compress $\mathcal{X}$ using $(\bm{U},\bm{V},\bm{W})$,
%\ENDFOR
%\label{code:fram:factorization}
%\label{code:fram:join}
%\STATE $(\bm{A}^{'},\bm{B}^{'},\bm{C}^{'})$ $\gets$ rank-R CP decomposition of $\mathcal{Y}$ via Alg. %\ref{alg:baseline CP},
%\STATE $\bm{A} \gets $ use OMP algorithm to solve for the $L_{1}$ constraint minimization problem %$\bm{A}^{'} = \bm{U}^{T}\bm{A}$, and likewise for $\bm{B}$ and $\bm{C}$, 
%\RETURN $(\bm{A}, \bm{B}, \bm{C})$. %算法的返回值
%\end{algorithmic}
%\end{algorithm}




%For the sparse tensors, the $\textit{exascale-tensor}$ scheme mainly consists of two stages, namely the compression stage same as that in the $\textit{exascale-tensor}$ scheme for dense tensors but here only one replica being created, i.e. $P=1$, and factorization stage is composed of CP decomposition of replica  and recovery of factorization matrices for raw data. 

%The difference for  sparse tensor decomposition in \textit{exascale-tensor} mainly in the factorization stage. To solve $\bm{A}=\mathop{\arg\min}_{\bm{A}} {\Vert \bm{A'}-\bm{U}\bm{A} \Vert}_{2}$ and likewise for $\bm{B}$ and $\bm{C}$, where ($\bm{A'},\bm{B'},\bm{C'}$) is the factorization matrix of the replica, different from the solving a least square problem for dense tensor decomposition, here, we fully utilize the sparsity of the raw tensor and its factorization matrix, view the $L_{2}$ minimization problem as a $L_{1}$ constraint minimization problem $\bm{A}=\mathop{\arg\min}_{\bm{A}} {\Vert \bm{A'}-\bm{U}\bm{A} \Vert}_{1}$. Here, we exploit  OMP-Cholesky  algorithm to solve the sparse-constraint least square problem to obtain $\bm{A}$ and likewise for $\bm{B}$ and $\bm{C}$.  

%The pseudocode for sparse tensor decomposition is shown in Alg. \ref{alg:Framworkforsparse}. From line $1$ -- $2$, the raw data $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$ is compressed into one replica $\mathcal{Y} \in \mathbb{R}^{L \times M \times N}$.  We use ALS to optimize  CP decomposition in Line $3$ and we utilize error-constraint OMP-Cholesky algorithm. 



%\subsection{Handing More Large Scale Sparse Tensors}

%Compared with the trillion-tensor scheme for dense condition, the scheme for sparse condition enjoys a much more efficiency due to the reduced cost of the compressed replicas, but it can not afford a arbitrary high compression rate which depends on the properties of the compression sense algorithm used. Thus,  to handle the large scale sparse tensors in our trillion-tensor scheme for sparse conditions, the bottleneck falls on the factorization of the compression replicas which might exceeds the maximum computation capacity of the CP decomposition. Here, we propose the embedded $\textit{Twice-Compression}$ method to combine the solutions for dense condition with sparse condition to handle more large scale sparse tensors with less efficiency loss. 

%Consider a large scale sparse tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$, for sparse condition, we compress it into the relative small tensor $\mathcal{Y} \in \mathbb{R}^{L \times M \times N}$ but it still exceeds the maximum computation capacity of CP decomposition. Note that the compression replica $\mathcal{Y}$ is usually dense, so we can exploit the trillion-tensor scheme for dense condition to run the tensor decomposition and obtain the factorization mode matrices of the compression replica. Then, we exploit the OMP algorithm to further recover the factorization mode matrices of the large scale tensor from the compression space.  

%Due to the property of the kronecker product, we have 
%\begin{equation}
%\label{compress twice process}\begin{split}
%    \bm{y}&=\textbf{Vec}(\mathcal{Y})\\
%    &=({\bm{U}_{p}}\otimes{\bm{V}_{p}}\otimes{\bm{W}_{p}})((\bm{U}\bm{A})\odot(\bm{V}\bm{B})\odot(\bm%{W}\bm{C}))\\
%    &=(({\bm{U}_{p}}\bm{U}\bm{A})\odot({\bm{V}_{p}}\bm{V}\bm{B})\odot({\bm{W}_{p}}\bm{W}\bm{C}))\\
%    &=(\hat{\bm{U}_{p}}\bm{A})\odot(\hat{\bm{V}_{p}}\bm{B})\odot(\hat{\bm{W}_{p}}\bm{C}),
%\end{split}
%\end{equation}
%where $\bm{U}_{p}$ is the random mode matrix for the first compression stage while $\hat{\bm{U}}$ is for the second compression stage, likewise for $(\bm{V}_{p},\hat{\bm{V}})$ and $(\bm{W}_{p},\hat{\bm{W}})$. Thus, the second time of  the compression stage is implicit that we can pre-process the random mode matrices by multiplying the corresponding random compression matrices of two stages with each other.


%Exploiting the feature that the compression replica at the begginning of  the implicit , the embedded $\textit{Twice-Compression}$ method for sparse condition actually obtain an extra compression rate income.  Compared with directly exploiting the scheme for dense condition, it demands for much fewer compression replicas. Thus, the $\textit{Twice-Compression}$ method can address the trouble for the limitations of the CP decomposition with the compression replica,  achieve the more large scale  sparse tensor decomposition. The reduction for the size for compression replicas also speedup the factorization stage. A proper setting of the compression rates for the twice compression can achieve the balance of the high efficiency and large computation capacity.  


%\begin{algorithm}[t] 
%\caption{Embedded Twice-Compression Trillion-Tensor %Scheme} 
%\label{alg:Twice compression Framwork} 
%\begin{algorithmic}[1] %这个1 表示每一行都显示数字
%\REQUIRE ~~\\ %算法的输入参数：Input
%tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times %K}$ with rank F; dimensions of first compression %replicas, $L, M, N$;dimensions of second compression %replicas, $qL, qM, qN$; the number of replicas $P$; the %number of common columns $S$.
%\ENSURE %算法的输出：Output
%mode matrices $(\bm{A}, \bm{B}, \bm{C})$;\\
%%\STATE Randomly generate matrices $\bm{U}_{p} \in %\mathbb{R}^{qL \times L},\bm{V}_{p} \in \mathbb{R}^{qM %\times M},\bm{W}_{p} \in \mathbb{R}^{qN \times N}$, %$p=1,2, .., P$, and set the first $S$ columns the same, %and randomly generate matrices $\bm{U} \in \mathbb{R}^{L %\times I},\bm{V} \in \mathbb{R}^{M \times J},\bm{W} \in %\mathbb{R}^{N \times K}$,
%\label{ code:fram:compression %}%对此行的标记，方便在文中引用算法的某个步骤
%\FOR{$p=1$ to $P$}
%\STATE $\mathcal{Y}_{p} \gets$ compress $\mathcal{X}$ %using $(\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{V},\bm{W}_{p}\bm{%W})$ , for $p = 1, .., P$,
%\ENDFOR
%\label{code:fram:factorization}
%\STATE $(\bm{A}^{'},\bm{B}^{'},\bm{C}^{'})$ $\gets$ run %the decomposition stage of rank-F compressed based CP %decomposition of $\{\mathcal{Y}_{p}\},p=1,2,...,P$,
%\STATE $\bm{A} \gets $ use OMP algorithm to solve for %the $L_{1}$ constraint minimization problem $\bm{A}^{'} %= \bm{U}\bm{A}$, and likewise for $\bm{B}$ and $\bm{C}$,
%\label{code:fram:join}

%\RETURN $(\bm{A}, \bm{B}, \bm{C})$. %算法的返回值
%\end{algorithmic}
%\end{algorithm}

%For instance, to handle a large scale sparse tensor $\mathcal{X} \in \mathbb{R}^{6,000 \times 6,000 \times 6,000}$,  in our trillion-tensor scheme for dense tensor, we can compress the large scale tensor into a series of relative  small  compression replicas $\mathcal{Y}_{p} \in \mathbb{R}^{200 \times 200 \times 200},p=1,2,...,30$ for simplify computation which occupied the memory of $30\times 200 \times 200 \times 200$ elem data types. When exploiting the sparse scheme, there is one relative large scale  compression replica $\mathcal{Y} \in \mathbb{R}^{600 \times 600 \times 600}$ which occupied the memory of $600 \times 600 \times 600$ elem data types. For the embedded $\textit{Twice-Compression}$ method, we can set the implicit number of replicas, $P=3$, for the second compression stage. And we will have $3$ replicas $\mathcal{Y}_{p} \mathbb{R}^{200 \times 200 \times 200}$, $p=1,2,3$, need to be factorized. And the demand memory is $3 \times 200 \times 200 \times 200$ elem data types. The embedded $\textit{Twice-Compression}$ method costs memory  $9\times$ less than the direct method for sparse condition and $10\times$ less than the method for dense condition. Correspondingly, the smaller size  and fewer number of the compression replicas will further accelerate the algorithm compared with the direct method for sparse and dense conditions. 

%\subsection{Multi-GPU Trillion-Tensor Scheme}
%We design a multi-GPU scheme for exascale-scale CP tensor decomposition to fully utilize the multiple GPUs in the computing device. Benefit from the property of the tensor contraction and spliting strategy used in the compression stage, the compression of each tensor block is independent of each other. And for muli-replicas conditions in our algorithm, i.e. dense condition and more large scale spase condition, there are multiple replicas need to be factorized and the decomposition of each  replica is also independent of each other. Thus, we can distribute the computation among multiple GPUs to compute in parallel. Suppose there are $c$ GPUs, denoted as $GPU_{1}$, ..., $GPU_{c}$, in the given computing device and the size of tensor is $I \times J \times K$. We set the size of block read in RAM one time is $B_{1 \times B_{2} \times B_{3}}$ and the number of total blocks $N=\frac{I \times J \times K}{B_{1} \times B_{2} \times B_{3}}$. We perform the parallel computation as follows:

%\begin{itemize}
    %\item CPU calculates and prepares the offset address of each block, $Addr_{1}, ..., Addr_{N}$, %then distributes them to a series of sets $C_{1}, ..., C_{c}$ of which number is related to the %number of GPUs and lastly send the sets to corresponding GPUs. The number of Address of each set %$\vert C_{i} \vert$ is proportional to the performance  of the $GPU_{i}$, $i=1, ..., c$, and we %have $\sum\limits_{i=1}^{c}\vert C_{i} \vert = N$.     
%    
 %   \item $GPU_{i}$ receives the to-be-processed address set $C_{i}$, and sequentially compress the %block referenced by the given set. For multi-replica conditions, to maximize the utilization of GPU, %we exploited the batch matrix multiplication to compress the block to multiple blocks in parallel. %The process of reading block is asynchronous between different GPUs which means that only one GPU %can access the data at the same time. Upon completion, the direct GPU to GPU communication will be %launched to send the result of $GPU_{i}$ to $GPU_{1}$ to form the final result.
 %   
  %  \item The following steps depends on the number of replicas.
   % \begin{itemize}
    %    \item For one replica condition, $GPU_{1}$ factorize the compressed tensor and the recovery %stage will be launched to obtain the estimation of the  mode matrices.
     %   
      %  \item For multi-replica condition, $GPU_{1}$ will construct a series of set $C_{1}, ..., %C_{c}$ of which set contains a number of replicas. Likewise, $C_{i}$ is is proportional to the %performance  of the $GPU_{i}$, $i=1, ..., c$. $GPU_{1}$ distributes the sets to corresponding %GPU and each GPU independently factorizes the compressed replicas. Upon completion, the results %from all GPUs will be merged to $GPU_{1}$ and $GPU_{1}$ continue to carry out the following %recovery stage to obtain the estimated mode matrices. 
    %\end{itemize}
%\end{itemize}
%The scheme fully utilize the advantages of multiple GPUs and independence of key operations in the algorithm  to accelerate the overall computation. The  data, except the address sets, transfer from GPU to GPU and no intermediate variables transferred back to CPU for reducing communication cost. And the direct GPU to GPU communication can be implemented by the memory copying routine supplied by the pyCUDA library.

==> The_Proposed_Solution.tex <==
\section{Exascale CP Tensor Decomposition}
\label{SEC_IMPLEMENTATION}

\begin{algorithm}[t] 
\caption{Exascale-Tensor Scheme} 
\label{alg:Twice compression Framwork} 
\begin{algorithmic}[1] %这个1 表示每一行都显示数字
\REQUIRE ~~\\ %算法的输入参数：Input
sparse tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$ with rank F; dimensions of first compression replicas, $L, M, N$;dimensions of second compression replicas, $qL, qM, qN$; the number of replicas $P$; the number of common columns $S$.
\ENSURE %算法的输出：Output
matrices $(\bm{A}, \bm{B}, \bm{C})$.\\
\STATE Randomly generate matrices $\bm{U}_{p} \in \mathbb{R}^{qL \times L},\bm{V}_{p} \in \mathbb{R}^{qM \times M},\bm{W}_{p} \in \mathbb{R}^{qN \times N}$, $p=1,2, .., P$, and set the first $S$ columns the same, and randomly generate matrices $\bm{U} \in \mathbb{R}^{L \times I},\bm{V} \in \mathbb{R}^{M \times J},\bm{W} \in \mathbb{R}^{N \times K}$,


\STATE $\mathcal{Y}_{p} \gets$ compress $\mathcal{X}$ using $(\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{V},\bm{W}_{p}\bm{W})$ according to  Eq. (\ref{compression_equation}), for $p = 1, .., P$,
%\ENDFOR
\label{code:fram:factorization}
\FOR{$p=1$ to $P$} 
\STATE $(\bm{A}_{p}, \bm{B}_{p}, \bm{C}_{p})$ $\gets$ rank-R CP decomposition  of $\mathcal{Y}_{p}$ via Alg. \ref{alg:baseline CP},
\STATE $(\bm{A}_{p},\bm{B}_{p},\bm{C}_{p})\gets$  divide each column of $(\bm{A}_{p},\bm{B}_{p},\bm{C}_{p})$ by the maximum of the first $S$ rows, respectively,
%\STATE $\Bar{\bm{A}_{p}}$ $\gets$ the first S rows of $\bm{A}_{p}$,
\STATE $\bm{\Pi}_{p}$ $\gets$  $\arg\max_{\bm{\Pi}} \text{Tr}(\bm{A}_{1}(1:S, :)^{T}\bm{A}_{p}(1:S, :)\bm{\Pi})$,
\STATE $(\bm{A}_{p},\bm{B}_{p},\bm{C}_{p}) \gets$  $(\bm{A}_{p}\bm{\Pi}, \bm{B}_{p}\bm{\Pi}, \bm{C}_{p}\bm{\Pi})$,
\ENDFOR
\label{code:fram:join}
\STATE $(\bm{A}^{*}, \bm{B}^{*}, \bm{C}^{*})$ $\gets$ solve  the least squares problem (\ref{lsq}) per mode,
\STATE $(\hat{\bm{A}},\hat{\bm{B}},\hat{\bm{C}})$ $\gets$ rank-R CP decomposition of $\mathcal{B}_{1}$,
\STATE $\bm{\Pi},\bm{\Sigma}$ $\gets$ match $\hat{\bm{A}}$ with the first $d_{1}$ rows of $\bm{A}^{*}$ using the Hungarian algorithm.
\STATE $\bm{A}^{'}$ $\gets$ $\bm{A}^{*}\bm{\Pi}\bm{\Sigma}$,
\STATE Repeat line 11-12 for $\bm{B}^{'}$ and $\bm{C}^{'}$, respectively,
\STATE $\bm{A} \gets $ use OMP algorithm to solve for the $L_{1}$ constraint minimization problem $\bm{A}^{'} = \bm{U}\bm{A}$, and likewise for $\bm{B}$ and $\bm{C}$,
\label{code:fram:join}

\RETURN $(\bm{A}, \bm{B}, \bm{C})$.
\end{algorithmic}
\end{algorithm}


In this section, we first demonstrate the motivation,  then present the \textit{Exascale-Tensor} for large-scale CP decomposition. 

\subsection{Overview}

% 用词需要统一  名词  动词 需要一致 
\begin{figure*}[t]
    \centering
    \includegraphics[height = 5cm, width = 18cm]{Figures/modify.jpg}
    \caption{Overview of the proposed \textit{Exascale-Tensor} decomposition, where the tensor $\mathcal{X} \in \mathbb{R}^{300 \times 300 \times 300}$, the amount P of the compression replicas $\mathcal{Y}$ is 8 $\ge \max(\frac{300-2}{50-2},\frac{300}{50},\frac{300}{50})$.}
    \label{pic_one-parallelization-schemes}
\end{figure*}



The \textit{Exascale-Tensor} algorithm mainly consists of of four stages, namely compression stage, factorization stage, recovering permutation and scaling stage, and compression sensing stage as shown in Fig. \ref{pic_one-parallelization-schemes}. The pseudo code  for \textit{Exascale-Tensor} is shown in Alg. \ref{alg:Twice compression Framwork}.


% 对应着图上的阶段名字
% 先讲图，再讲算法，算法第几行到第几行对应哪部分....

%First, a tensor $\mathcal{X} \in \mathbb{R}^{300 \times 300 \times 300}$, consisting of $27$ tensor blocks $\mathcal{B}_{n} \in \mathbb{R}^{100 \times 100 \times 100}$, $n=1, 2, ..., 27$, is first compressed into $8$ replicas $\mathcal{Y}_{p} \in \mathbb{R}^{50 \times 50 \times 50}$, $p=1, 2, ..., 8$. Second, using CP decomposition, each replica is factored to matrices independently. Thirdly, with a proper permutation and normalization, solving a least squares problem for each mode will result in the factorization matrices $(\bm{A}^{*},\bm{B}^{*},\bm{C}^{*})$. Using the factorization of the first block $\mathcal{B}_{1}$, we get the permutation matrix $\bm{\Pi}$ and the scaling matrix $\bm{\Sigma}$. Then, we use $\bm{\Pi}$ and $\bm{\Sigma}$ to obtain the full mode matrices $(\bm{A},\bm{B},\bm{C})$. 

%First, a tensor $\mathcal{X} \in \mathbb{R}^{200 \times 200 \times 200}$ of rank $5$, is divided into $8$ blocks $\mathcal{B}_{n} \in \mathbb{R}^{100 \times 100 \times 100}$, $n=1, 2, ..., 8$, and then  compressed into $3$ replicas $\mathcal{Y}_{p} \in \mathbb{R}^{50 \times 50 \times 50}$, $p=1, 2, 3$, where the $n$-th block $\mathcal{B}_{n}$ is compressed into $\mathcal{Y}_{p}^{n}$ by $\bm{U}_{p},\bm{V}_{p}$  and $\bm{W}_{p}$ which are the generated random compression matrices introduced in Section \ref{compression_based_demo}, and $\mathcal{Y}_{p}=\sum\limits_{n}\mathcal{Y}_{p}^{n}$, $p=1, 2, 3$, $n=1, 2, ..., 8$.

First,  a sparse tensor $\mathcal{X} \in \mathbb{R}^{300 \times 300 \times 300}$ of rank $5$, is divided into $27$ blocks $\mathcal{B}_{n} \in \mathbb{R}^{100 \times 100 \times 100}$, $n=1, 2, ..., 27$. Each block $\mathcal{B}_{n}$ will be compressed $8$ times by $\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{V}$ and $\bm{W}_{p}\bm{W}$, where $\bm{U}_{p}, \bm{V}_{p},\bm{W}_{p} \in \mathbb{R}^{50 \times 80}$, $p=1, 2, .., 8$, and  $\bm{U}, \bm{V}, \bm{W} \in \mathbb{R}^{80 \times 100}$, which are the generated random compression matrices introduced in Section \ref{compression_based_demo}.   Specifically, the $n$-th block $\mathcal{B}_{n}$ is compressed into $\mathcal{Y}_{p}^{n}$, $p=1,2,..., 8$. Then, by 
adding all the $p$-th replicas of each block,  we can get the $p$-th replica of the original tensor $\mathcal{X}$,  $\mathcal{Y}_{p}$.  That is,  $\mathcal{Y}_{p}=\sum\limits_{n}\mathcal{Y}_{p}^{n}$,   $p=1, 2,..., 8$,  $n=1, 2, ..., 27$,  $\mathcal{Y}_{p} \in \mathbb{R}^{50 \times 50 \times 50}$.

Second, using CP decomposition, each replica $\mathcal{Y}_{p}$ is factored to matrices, $\bm{A}_{p} \in \mathbb{R}^{50 \times 5}$, $\bm{B}_{p} \in \mathbb{R}^{50 \times 5}$,  $\bm{C}_{p} \in \mathbb{R}^{50 \times 5}$, $p=1, 2,..., 8$. Note that the compression of $\mathcal{X}$ by $\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{V}$ and $\bm{W}_{p}\bm{W}$, can be written as
\begin{equation}
\begin{split}
    \bm{y}_{p}&=\text{Vec}(\bm{Y}_{p})\\
    &=(({(\bm{U}_{p}\bm{U})}\otimes{(\bm{V}_{p}\bm{V})}\otimes{(\bm{W}_{p}\bm{W})})(\bm{A}\odot\bm{B}\odot\bm{C}))\bm{1}\\
    &=((\bm{U}_{p}\bm{U}\bm{A})\odot(\bm{V}_{p}\bm{V}\bm{B})\odot(\bm{W}_{p}\bm{W}\bm{C}))\bm{1},
\end{split}
\end{equation}
 where $\bm{A}, \bm{B}$ and $\bm{C}$ are the factorization matrices of $\mathcal{X}$. According to the definition of CP decomposition, the factorization of the replica $\mathcal{Y}_{p}$ can be written as 
 \begin{equation}
 \begin{split}
 \bm{y}_{p}=(\bm{A}_{p}\odot\bm{B}_{p}\odot\bm{C}_{p})\bm{1}
 \end{split}
 \end{equation}
 Therefore, due to the uniqueness of CP decomposition up to scaling and permutations, we have 
 \begin{equation}
 \begin{split}
 \bm{A}_{p}&=\bm{U}_{p}\bm{U}\bm{A}=\bm{U}_{p}\bm{U}\bm{A}\bm{\Pi}_{p}\bm{\Sigma}_{p}^{a},\\
 \bm{B}_{p}&=\bm{V}_{p}\bm{V}\bm{B}=\bm{V}_{p}\bm{V}\bm{B}\bm{\Pi}_{p}\bm{\Sigma}_{p}^{b},\\
 \bm{C}_{p}&=\bm{W}_{p}\bm{W}\bm{C}=\bm{W}_{p}\bm{W}\bm{C}\bm{\Pi}_{p}\bm{\Sigma}_{p}^{c}
 \end{split}
 \end{equation}
 where $\bm{A}, \bm{B}, \bm{C}$ are the CP factorization matrices of $\mathcal{X}$ as shown in Eq. (\ref{cp_equation}), $\bm{\Pi}_{p}$ is the column permutation matrix, $\bm{\Sigma}_{p}$ is the column scaling matrix and $\bm{\Sigma}_{p}^{a}\bm{\Sigma}_{p}^{b}\bm{\Sigma}_{p}^{c}=\bm{I}$. Using Hungarian algorithm and dividing by the maximum elem in each column, the factored matrices have a common permutation and scaling which satisfy 
 \begin{equation}
 \begin{split}
 \bm{A}_{p}&=\bm{U}_{p}\bm{U}\bm{A}\bm{\Pi}\bm{\Sigma}^{a},\\  \bm{B}_{p}&=\bm{V}_{p}\bm{V}\bm{B}\bm{\Pi}\bm{\Sigma}^{b},\\ \bm{C}_{p}&=\bm{W}_{p}\bm{W}\bm{C}\bm{\Pi}\bm{\Sigma}^{c}. 
 \end{split}
 \end{equation}
 Then, using a least square method for each mode will result in the factorization matrix $\bm{A}^{*},\bm{B}^{*}$ and $\bm{C}^{*}$ which satisfy
 \begin{equation}
\begin{split}
 \bm{A}^{*}&=\bm{U}\bm{A}\bm{\Pi}\bm{\Sigma}^{a}, \\ \bm{B}^{*}&=\bm{V}\bm{B}\bm{\Pi}\bm{\Sigma}^{b},\\  \bm{C}^{*}&=\bm{W}\bm{C}\bm{\Pi}\bm{\Sigma}^{c}.
\end{split}
\end{equation}
Third, because of the uniqueness of CP decomposition, using the factorization of a compression replica for the first block $\mathcal{B}_{1}$ using $\{\bm{U}, \bm{V}, \bm{W}\}$, we can get the permutation matrix $\bm{\Pi}$ and the scaling matrices $\bm{\Sigma}^{a}$, $\bm{\Sigma}^{b}$ and $\bm{\Sigma}^{c}$. We use  the permutation and scaling matrices  to obtain $(\bm{A'},\bm{B'},\bm{C'})$, where we have
\begin{equation}
\label{last equation}
\begin{split}
\bm{A'}&=\bm{U}\bm{A}\\
\bm{B'}&=\bm{V}\bm{B}\\
\bm{C'}&=\bm{W}\bm{C}    
\end{split}
\end{equation}
Last, exploiting the sparsity of $\mathcal{X}$, we use OMP algorithm to solve the $L_{1}$ constraint minimization problems as shown in Eq. (\ref{last equation}), and obtain the full mode matrices $\bm{A}$, $\bm{B}$ and $\bm{C}$. 


%Thirdly, after a proper permutation and scaling for columns  of factored matrices, solving a least squares problem for each mode will result in the factorization matrices  $(\bm{A}^{*},\bm{B}^{*},\bm{C}^{*})$. Using the factorization of the first block $\mathcal{B}_{1}$, we get the permutation matrix $\bm{\Pi}$ and the scaling matrix $\bm{\Sigma}$. Then, we use $\bm{\Pi}$ and $\bm{\Sigma}$ to obtain the full mode matrices $(\bm{A},\bm{B},\bm{C})$.



%For the sparse tensors, the $\textit{trillion-tensor}$ algorithm mainly consists of two stages, namely the compression stage same as that in the $\textit{trillion-tensor}$ algorithm for dense tensors but here only one replica being created, and factorization stage composed of tensor decomposition in compressed domain and recovery of mode matrices in uncompressed space as given in Alg. \ref{alg:Framworkforsparse}. It differs from the algorithm for dense tensors mainly in the factorization stage which it utilizes the compressed sensing theory to directly solve the sparsity-constrained linear system per-mode for restoring the mode matrices in uncompressed space. 








% 点名计算任务

\subsection{Compression Stage}

The compression stage is corresponding to line 1--2  in  Alg. \ref{alg:Twice compression Framwork}. To compress tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$ into $\mathcal{Y} \in \mathbb{R}^{L \times M \times N}$, the $(i,j,k)$-th element of $\mathcal{Y}$ is computed as follows: 
\begin{equation}
\label{compression_equation}
    \mathcal{Y}_{lmn}=\sum\limits_{i=1}^{I}\sum\limits_{j=1}^{J}\sum\limits_{k=1}^{K}\bm{U}_{li}\bm{V}_{mj}\bm{W}_{nk}\mathcal{X}_{ijk},
\end{equation}
where $\bm{U}\in\mathbb{R}^{L \times I} , \bm{V}\in\mathbb{R}^{M \times J}, \bm{W}\in\mathbb{R}^{N \times K}$ are random matrices from the normal distribution. %It can be seen as an iterative steps: reshape $\bm{U}^{T}\bm{X}_{(1)}$ to $\mathcal{G} \in \mathbb{R}^{L \times J \times K}$, then reshape $\bm{W}^{T}\bm{G}_{(3)}$  to $\mathcal{G} \in \mathbb{R}^{L \times J \times N}$, and finally reshape $\bm{V}^{T}\bm{G}_{(2)}$ to $\mathcal{Y}$ as we wanted.

In \textit{Exascale-Tensor}, $\mathcal{X}$ will be compressed twice. \mathcal{X} is first compressed into one relative small replica $\mathcal{Y} \in \mathbb{R}^{L \times M \times N}$. Then $\mathcal{Y}_{p}$ will be compressed  into P replicas $\mathcal{Y}_{p} \in \mathbb{R}^{qL \times qM \times qN}$, $p=1,2,...,P$,  $P \ge \max(\frac{L-2}{qL-2},\frac{M}{qM},\frac{N}{qN})$. Two continuous compression can be  equivalent to  one time of compression for $\mathcal{X}$ using $(\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{V},\bm{W}_{p}\bm{W})$.



%While for the sparse tensors, there is only one replica needed, i.e., $P=1$, but the compression rate will be constrained due to the compressed sensing theory, $I \gg L > 2K_{A}$, where $K_{A}$ is the latent sparsity of the load matrix $\bm{A}$ along the I-mode of the tensor, and likewise for the J-mode and K-mode. 




To process an ``out-of-memory" tensor, we adopt a spliting  strategy that we first split $\mathcal{X}$ into multiple blocks $\mathcal{B}_{n} \in \mathbb{R}^{d_{1} \times d_{2} \times d_{3}}$ $n=1,2,...,\frac{IJK}{d_{1}d_{2}d_{3}}$ as shown for example in Fig.  \ref{pic_one-parallelization-schemes}. Then, due to the block tensor operation, we exploit the related components of $(\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{U},\bm{W}_{p}\bm{W})$ to compress each block $\mathcal{B}_{n}$ to replicas $\mathcal{Y}_{p}^{n}$, $p=1,2,...P$, where $\bm{U}_{p} \in \mathbb{R}^{qL \times L}$, $\bm{V}_{p} \in \mathbb{R}^{qM \times M}$, $\bm{W}_{p} \in 
\mathbb{W}_{p} \in \mathbb{R}^{qN \times N}$ and $\bm{U} \in \mathbb{R}^{L \tiems I}$, $\bm{V} \in \mathbb{R}^{M \times J}$,  $\bm{W} \in \mathbb{R}^{N \times K}$, $P \ge \max(\frac{L-2}{qL-2},\frac{M}{qM},\frac{N}{qN})$, $L \ge 2K_{A}$, $M \ge 2K_{B}$ $N \ge 2K_{C}$, $\{K_{A},K_{B},K_{C}\}$ denoted as the latent sparsity of $\mathcal{X}$ along each mode respectively. Finally,  accumulate them to the final replicas $\mathcal{Y}_{p}$ respectively, i.e.,  $\mathcal{Y}_{p}+=\mathcal{Y}_{p}^{n}$,   $p=1,2,..,P$.
% Different from directly using $\{\bm{U}_{p},\bm{V}_{p},\bm{W}_{p}\}$ in \textit{Trillion-Tensor}, we use   $\{\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{V},\bm{W}_{p}\bm{W}\}$ to compress the large tensor. The  use of additional matrix further improve the compression ratio and exploiting the latent sparsity of $\mathcal{X}$ for following compression sensing stage.



%The essential of the compression stage is to multiply every slab of the tensor $\mathcal{X}$ from the I-mode with $\bm{U}_{p}^{T}$, the J-mode with $\bm{V}_{p}^{T}$ and the K-mode with $\bm{W}_{p}^{T}$. To address the terrible situation that we can not load the full large tensor $\mathcal{X}$ into RAM, we adopt the strategy that we first split the large tensor into some  tensor blocks $\mathcal{B}_{n} \in \mathbb{R}^{d_{1} \times d_{2} \times d_{3}}$ with the number of $\frac{I \times J \times K}{d_{1} \times d_{2} \times d_{3}}$ as shown for example in Figure \ref{pic_one-parallelization-schemes}, then multiply each tensor block $\mathcal{B}_{n}$ read in RAM with corresponding mode compression sub-matrices  to get one component of the replica $\mathcal{Y}_{p}^{\mathcal{B}_{n}}$, and finally accumulate it to the final replica $\mathcal{Y}_{p}$.
   

\subsection{Factorization Stage}

The factorization stage is  involved in line 3--9 of Alg. \ref{alg:Twice compression Framwork}. On the factorization stage, each replica $\mathcal{Y}_{p}$ will be independently factored to $(\bm{A}_{p},\bm{B}_{p},\bm{C}_{p})$, $p=1,2,..,P$, using the CP decomposition shown in Alg.\ref{alg:baseline CP}. Due to a property of the Kronecker product \cite{kr_property}, we have the equation $\bm{A}_{p}=\bm{U}_{p}\bm{U}\bm{A}\bm{\Pi}_{p}\bm{\Sigma}_{p}$,  $p=1,2,...,P$.  Here, we apply Hungarian algorithm \cite{HA} to  the trace maximization problem to get rid of $\bm{\Pi}_{p}$ and divide each column by  its maximum of the first S rows to get rid of $\bm{\Sigma}_{p}$, where we $S$ is the number of shared columns in the random matrices $\bm{U}_{p}, p=1,2,...,P$. Finally, solve a master least squares problem 
\begin{equation}
\label{lsq}
\left[
\begin{array}{c}
     \bm{A}_{1}\\
     \vdots    \\
     \bm{A}_{P}\\
\end{array}
\right]
=
\left[
\begin{array}{c}
    \bm{U}_{1} \\ 
    \vdots    \\
    \bm{U}_{P}
\end{array}
\right]
\bm{U}\bm{A}\bm{\Pi}\bm{\Sigma}
\end{equation}
to obtain $\bm{A}^{*} =\bm{U}\bm{A}\bm{\Pi}\bm{\Sigma}$,  and similarly for $\bm{B}^{*}$ and $\bm{C}^{*}$.

%For sparse tensors, on the factorization stage, the replica $\mathcal{Y}$ will be first factored to $(\bm{A}_{y},\bm{B}_{y},\bm{C}_{y})$. Due to a property of the Kronecker product, we have the constraint $\bm{A}_{y}=\bm{U}^{T}\bm{A}$. Different from the solution for dense tensors, the load matrix $\bm{A} \in \mathbb{R}{I \times F}$ is sufficiently sparse with supposed sparsity  $K_{A}$, with the projection matrix $\bm{U} \in \mathbb{R}^{L \times I}$ which satisfies $I \gg L > 2K_{A}$. Thus, this problem can be rewritten as an classical $l_{0}$ constraint minimization problem
%\begin{equation}
%\label{compression_equation_for_sparse}
%    \min\limits_{A}{\Vert\bm{A}_{y}-\bm{U}\bm{A}\Vert}_{%2}^{2} \textit{ subject to }  {\Vert\bm{A}\Vert}_{0} %\leq K_{A},
%\end{equation}

%where ${\Vert\bm{A}\Vert}_{0}$ is the $L_{0}$ pseudo-norm, i.e. the number of nonzero elements in $\bm{A}$.  According to the compressed sensing theory, it is natural to regard $\bm{A}$ as the latent sparse signals in high-dimension uncompressed space, $\bm{U}$ as the dictionary, and $\bm{A}_{y}$ as the observation signals in low-dimension compression domain. Here, we exploit  OMP-Cholesky  algorithm to solve the sparse-constraint least square problem to obtain $\bm{A}$ and likewise for $\bm{B}$ and $\bm{C}$.  

\subsection{Recovering Scaling and Permutations}

The recovering scaling and permutation stage is involved in line 10--13 of Alg. \ref{alg:Twice compression Framwork}. To recover the scaling and permutations, we use the factors $(\hat{\bm{A}},\hat{\bm{B}},\hat{\bm{C}})$ of the compression replica for first block $\mathcal{B}_{1}$ using $\{\bm{U},\bm{V},\bm{W}\}$ as compression matrices. Because the CP tensor decomposition is unique, we assume that $(\hat{\bm{A}},\hat{\bm{B}},\hat{\bm{C}})$ are the first $d_{1}$ rows of full mode matrices $(\bm{A}^{*},\bm{B}^{*},\bm{C}^{*})$, i.e., $\hat{\bm{A}}={\bm{A}^{*}}(1:d_{1},:)\bm{\Pi}\bm{\Sigma}$. Here, we make the diagonal entries of the scaling  matrix $\bm{\Sigma}$ composed of  the maximums of each column in $\hat{\bm{A}}$, i.e. $\bm{\bm{\Sigma}}=\text{diag}( \max(\hat{\bm{A}}(:,1)), ..., \max(\hat{\bm{A}}(:,F) ) )$. To obtain  the full mode matrix $\bm{A}^{'}$  for the compression replica of $\mathcal{X}$ using $(\bm{U},\bm{V},\bm{W}$), first, we divide each column of $\hat{\bm{A}}$ by its maximum and divide each column of $\bm{A}^{*}$ by its maximum of the first $d_{1}$ rows.  Second,  similar to the factorization stage, we apply the Hungarian algorithm \cite{HA} to maximize $\text{Tr}({\hat{\bm{A}}}^{T}{\bm{A}^{*}}(1:d_{1},:)\bm{\Pi})$ and obtain the permutation matrix $\bm{\Pi}$. Thus, we get the mode matrix $\bm{A}^{'}=\bm{U}\bm{A}^{*}\bm{\Pi}\bm{\Sigma}$, similarly for $\bm{B}^{'}$ and $\bm{C}^{'}$.




%/In practice, we usually make the first block on this stage,  $\mathcal{B}_{1} \in \mathbb{R}^{d_{1} \times d_{2} \times d_{3}}$, to be different from that on the compression stage in the size. And in our experiment of the large-scale tensor decomposition, it is proved to be effective if we  set $d_{1} \neq d_{2} \neq d_{3}$ and make the size of the tensor block on current stage smaller than that on the compression stage when the rank $F$ of tensor $\mathcal{X}$ is relative smaller than the size of tensor. 




\subsection{Compression Sensing Stage}

The compression sensing stage corresponds to line 14 of Alg. \ref{alg:Twice compression Framwork}. 
Compression sensing can be formally described as 
\begin{equation}
    \bm{Y}=\bm{U}\bm{A},
\end{equation}
where $\bm{Y} \in \mathbb{R}^{L \times F}$ denoted as measurement matrix, $\bm{U} \in \mathbb{R}^{L \times I}$ denoted as the dictionary, $\bm{A} \in \mathbb{R}^{I \times F}$ denoted as the sparse   signal matrix. 

For $\bm{A'},\bm{B'}$ and $\bm{C'}$ obtained on the recovering stage and  we have $\bm{A'}=\bm{U}\bm{A}$, $\bm{B'}=\bm{V}\bm{B}$ and $\bm{C'}=\bm{W}\bm{C}$ where $\bm{A},\bm{B}$ and $\bm{C}$ are sparse. So, it is equivalent to the the compression sensing problem and  we can use $L_{1}$ constraint minimization algorithm OMP to solve the problems to obtain full mode matrices $\bm{A}$, $\bm{B}$ and $\bm{C}$.






%On the compression stage, the \textit{Exascale-Tensor} scheme reads block tensor from memory, alternatively utilize the tensor matricization and matrix multiplication in each axis to compress large tensor to small replicas. This process consists of data-independent operations including matrix transport, tensor matricization and matrix multiplication which are suitable for parallel computations.  

%Besides, the compression of all replicas and the decomposition of each replica is also independent with each other which is suitable for parallel computations.

%Thus, we propose to offload the data-independent and high parallel computations from CPU to GPU which is of effect for massive parallel computations.   We furthermore performed preliminary experiments to evaluate the GPU implementation of \texit{Trillion-Tensor}  and observed that low memory access efficiency, expensive device communication and low utilization of GPUs are the bottlenecks restricting the performance of our scheme. Therefore, we mainly focus on optimization these aspects in the following context. 




%The last stage is designed for mode estimation matrices $(\bm{A}^{*},\bm{B}^{*},\bm{C}^{*})$ to recover  the scaling and permutations.
%Resort to the uniqueness of CP tensor decomposition and the property of low rank for tensors, intuitively, for a given large tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$, we might as well assume the factorization mode matrices $(\bm{A}',\bm{B}',\bm{C}')$ of the sub tensor block $\mathcal{B}_{1}$, located in the first corner as shown for example in Figure \ref{pic_one-parallelization-schemes},  is same with the corresponding sub-matrices of the factorization mode matrices $(\bm{A},\bm{B},\bm{C})$ from the full tensor. 

%From this point of view, to recover from the permutations and scaling for mode estimation matrices we get on the factorization stage, we can make full use of the factorization result $(\bm{A}',\bm{B}',\bm{C}')$ of the tensor block $\mathcal{B}_{1}$. Due to the uniqueness of CP tensor decomposition and the property of low rank for tensors, we have the constraint equation $\bm{A}^{*}'= \bm{A}'\bm{\Pi}\bm{\Sigma}$ (likewise for $\bm{B}^{*}$ and $\bm{C}^{*}$), where $\bm{A}^{*}'$ is the corresponding sub-matrix of $\bm{A}^{*}$ related to $\bm{A}'$, and $\bm{\Pi}$, $\bm{\Sigma}$ are the permutation and scaling matrices. Similarly to the factorization stage, to get ride of the permutation matrix $\bm{\Pi}$, we apply the Hungarian algorithm for matching the normalized mode estimation sub matrix $\bm{A}^{*}'$ with the normalized $\bm{A}'$. After permutation, we multiply corresponding column factors of anchor mode matrices to normalized estimation matrices to get rid of the scaling matrix $\bm{\Sigma}$.

 




%\subsection{Optimizations}
%The computational complexity of the compression stage is $O(PIJK \times \min(L,M,N))$ versus $O(\frac{IJ}{F})$ of the factorization stage \cite{paracomp}.  Huge time consumption of the compression stage is the bottleneck of this algorithm with the size of tensor increasing.  

%On the compression stage, operations of all tensor blocks $\mathcal{B}_{n}, n=1, 2, ..., \frac{IJK}{d_{1}d_{2}d_{3}}$, are independent of each other, and the respective compression result $\mathcal{Y}_{p}^{n}$  will be accumulated to the  common replica $\mathcal{Y}_{p}$, $p=1,2,..., P$. There is $\frac{IJK}{d_{1}d_{2}d_{3}}$ parallelism in this process. Thus, we design two parallelization schemes for efficient compression on CPUs and GPUs, respectively. 


%\textbf{Parallel implementation on CPUs}: This scheme advocates exploiting the property of multi-core processors on CPUs. In this scheme, we compress the tensor block $\mathcal{B}_{n}$, $n=1,2,...,\frac{IJK}{d_{1}d_{2}d_{3}}$, in parallel on multi processes. On each sub-process, one of tensor blocks, $\mathcal{B}_{n}$, will be loaded in memory and  independently compressed into sub-replicas $\mathcal{Y}_{p}^{n}$, $p=1,2,...,P$, then the sub-replicas will be accumulated to corresponding common  replicas $\mathcal{Y}_{p}$ shared on the main process,  $p=1,2,...,P$.

%\textbf{Parallel implementation on GPUs}: 
%This scheme advocates exploiting GPUs' high performance in matrix multiplication. Consider a given situation that for a trillion-scale tensor $\mathcal{X} \in \mathbb{R}^{10,000 \times 10,000 \times 10,000}$ composed of tensor blocks $\mathcal{B}_{n} \in \mathbb{R}^{500 \times 500 \times 500}$, $n=1,2,...,8000$, there are    $3 \times 8,000$ times of matrix multiplication need to be done. The huge time consumption of extra large-scale matrix multiplication on CPUs is always unbearable. However, compared to CPU, GPU is more suitable for large-scale matrix multiplication for its much greater number of relatively unexceptional processing cores.

%Thus, compared to the parallel implementation on CPUs, this scheme differs only in the matrix computation step, in which it transfer the block $\mathcal{B}_{n}$ of each sub-process from CPUs to GPUs and the following compression steps except the accumulation will work on GPUs. The accumulation step will first transfer $\mathcal{Y}_{p}^{n}$, $p=1,2,...,P$ to CPUs and then accumulate them to corresponding replicas.


%Because of the parallelism of the multiplication of tensor blocks with related random mode sub-matrices $\bm{U}_{p}^{'}, \bm{V}_{p}^{'},\bm{W}_{p}^{'}$, in our work, we put the the compression of the tensor block $\mathcal{B}_{n}$ on multi processes, and set the replica set ${\{\mathcal{Y}_{p}\}}_{p=1,2,...,P}$ on the main process to be shared with sub-processes, i.e., on each process, we independently compress one tensor block $\mathcal{B}_{n}$ to a series of sub-replicas ${\{\mathcal{Y}_{p}^{\mathcal{B}_{n}}\}}_{p=1,2,...,P}$, and corresponding accumulate them to replicas set ${\{\mathcal{Y}_{p}\}}_{p=1,2,...,P}$ on the main process.


%Consider a given situation that for a trillion-scale tensor $\mathcal{X} \in \mathbb{R}^{1w \times 1w \times 1w}$ composed of tensor blocks $\mathcal{B}_{n} \in \mathbb{R}^{500 \times 500 \times 500}$, there are 8000 blocks need to be compressed and $3 \times 8000$ times of matrix multiplication need to be done. The huge time consumption of extra large-scale matrix multiplication on CPU is always unbearable. However, compared to CPU, GPU is more suitable for large-scale matrix multiplication for its much greater number of relatively unexceptional processing cores. Thus, in order to reduce the huge time consumption of the matrix multiplication, we exploit the characteristic of GPU on matrix multiplication tasks and take the strategy that load the tensor blocks  $\mathcal{B}_{n}$ into the video memory on GPUs in parallel, then compress it to sub-replicas ${\{\mathcal{Y}_{p}^{\mathcal{B}_{n}}\}}_{p=1,2,...,P}$ serially, and finally merge them to  ${\{\mathcal{Y}_{p}\}}_{p=1,2,...,P}$ on the main process. 

%Based on the complexity-order analysis of algorithm,  consider a situation where a big tensor $\mathcalc{X} \in \mathbb{R}^{I \times J \times K}$ and the compression replicas $\mathcalc{Y}_{p} \in \mathbb{R}^{L \times M \times N}$ with number of P, the complexity-order of the compression stage is $O(PIJK\times \min(L,M,N))$ versus $O(\frac{IJ}{F})$ for the factorization stage.  Huge time consuming of the compression stage is the bottleneck of this tensor decomposition algorithm with the size of tensor increasing.

%To reduce the huge time consumption of computation on the compression stage, we exploit the property of multi-cores on CPUs and the powerful matrix computation performance on GPUs,  developing two different acceleration frameworks on CPUs and GPUs respectively to make a preliminary acceleration.
%In our work, we make a preliminary acceleration with a parallel framework embedding in the stage of compressing the tensor block to P compressed tensor cubes, and make full use of high-performance computations for matrix operations on GPU, to as much as possible accelerate the procedure of super huge scale tensor decomposition.



%Specially, In the stage of tensor compression, we carefully design the size of tensor block read in RAM, and put it directly in GPU to be shared with multiple threads. And we directly take out the corresponding mode compression submatrices on GPU for each thread in parallel to reduce the time cost. These tricks reduce the huge time consuming on tensor compression significantly.    





==> dac24/Sections/Efficient.tex <==
\section{High Performance Exascale Implemetation}


In this section, we will first give an overall optimization on GPU implementation against the above parallel analysis, including designing efficient data storage, reducing communication overhead and improving  the utilization of GPUs. Then we will carefully design and implement optimization scheme on compression and decomposition stage respectively. 

%In this section, we will first give a roughly theoretical analysis of the maximum size of the tensors our methods supported, and show an feasible scheme for supporting exascale tensors. Then we will specifically point out the bottlenecks that limit the performance. Against the above analysis, we propose some optimization methods to improve the efficiency including optimizing the data storage, reducing communication overhead, improving the utilization of GPUs and so on. 



% In the following sections, we will focus on optimize data storage, device communications, key operations on each stage to design and implement an high performance \textit{trillion-tensor} scheme on GPU. 



%We profiled both the CPU Python implementations of our trillion-tensor scheme for dense and sparse tensorss, and found that the compression stage took most of the time of the total running time for  these algorithms with the size of tensors increasing, while for relative small sizes of tensors, the factorization stage was the bottleneck to limit the efficiency of the algorithms. Thus, for large scale tensors, we can significantly improve the performance on the compression stage to accelerate the trillion-tensor scheme both for dense and sparse tensors.

%On the compression stage, the algorithm scheme both for dense and sparse tensorss exploits the Equation (\ref{compression_equation}) to compress the large scale tensor to $P$ replicas, while for sparse tensors, $P=1$. It can be rewritten as the following iterative process:
%\begin{equation}
%\label{compress equal matrix}
%    \begin{split}
%        \mathcal{Y}&=\mathcal{X}\\
%        \bm{Y}_{(1)}&=\bm{U}\bm{X}_{(1)}\\
%        \bm{Y}_{(3)}&=\bm{W}\bm{Y}_{(3)}\\
%        \bm{Y}_{(2)}&=\bm{V}\bm{Y}_{(2)},
%    \end{split}
%\end{equation}
%with updating the replica $\mathcal{Y}$ and its matricization forms along all modes after each step. This process involves intensive computations and data transfer operations including matrix multiplication, tensor matricization and matrix folding. Compared to CPU, GPU is more suitable for large scale matrix multiplication and other data-independent operations for its much greater number of relatively unexceptional processing cores. For the factorization stage both for dense and sparse tensorss, iterative computations involved solve large scale linear square problems can also be significantly accelerated benefit from the perfect CUDA library in python. So we offload these computations in our scheme from CPU to GPU and focus on designing  and implementing our high performance trillion-tensor scheme on GPU. 



 
 
 
 
 %The data is default to computation in row-major format for the build-insert functions in Python  and supplied  APIs in Numpy. Thus, we store the data in row-major format. 
  
 %There is one disadvantage using this format that some routines in the pyCUDA libraries use the column-major format. The most time consuming key operation on the compression stage  is the matrix multiplication and it utilizes the cublasDgemm routine in pyCUDA library that uses  the column-major format. But the conflict can be solved by the latent matrix transpose with no additional compution and storage overhead. 
 
 %For example of the computation of $\bm{C}=\bm{A}\bm{B}$, due to the row-major storage format, the libraries actually take $\bm{A}^{T}$ and $\bm{B}^{T}$ as operand. Thus, we can transpose both the LHS and RHS to give $\bm{C}^{T}=\bm{B}^{T}\bm{A}^{T}$. Notice that there is no explicit matrix transpose, due to the $1D$ linear storage, $\bm{C}^{T}$ in column-major format is actually $\bm{C}$ in row-major format. The other operations depend on column-major used in CUDA libraries  consume less, the transformation of data storage format will not bring much consumption. Comprehensive consideration makes us adopt the row-major format.







\subsection{Optimization Compression Stage}

The compression process of tensor $\mathcal{X}$ for an replica $\mathcal{Y}_{p}$ for line 2 in Alg. \ref{alg:Twice compression Framwork} and Eq. \ref{compression_equation}  can be rewritten as following according to Eq. \ref{compression_equation},
\begin{equation}
    \label{compress equal matrix}\begin{split}
    \bm{y}_{p}&=\textbf{Vec}(\mathcal{Y}_{p})\\
    &=({\bm{U}_{p}}\otimes{\bm{V}_{p}}\otimes{\bm{W}_{p}})(\bm{A}\odot\bm{B}\odot\bm{C})\\
    &=((\bm{U}_{p}\bm{A})\odot(\bm{V}_{p}\bm{B})\odot(\bm{W}_{p}\bm{C})),
\end{split}
\end{equation}
where $\bm{U}_{p}, \bm{V}_{p}$ and $\bm{W}_{p}$ are the compression matrices to compress $\mathcal{X}$ to $\mathcal{Y}_{p}$, and $\bm{A}, \bm{B}$ and $\bm{C}$ are the latent decomposition factors of $\mathcal{X}$. i.e., $\textbf{Vec}(\mathcal{X})=(\bm{A}\odot\bm{B}\odot\bm{C})\bm{1}$.  Thus, the major computations involves three times of  matrix multiplications for every block on the computation stage. In the following sub-subsections, we mainly focus optimize the matrix multiplications on GPUs to accelerate the compression stage. 

\subsubsection{Efficient Compression Using Sparse Projection}

For the computation step in line 2 of Alg. \ref{alg:Twice compression Framwork}, we use the  random normal initialized matrix to compress the large scale tensor into small replicas. For each time of compression for one block, there exist $3$ times matrix multiplications shown in Eq.(\ref{compress equal matrix}), i.e., each time of matrix  multiplication corresponding to the compression for each dimension. Considering a tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$ and the compression replica $\mathcal{Y} \in \mathbb{R}^{L \times M \times N}$ where $I=J=K=500$ and $L=M=N=200$, take the first compression step  as example, we have the following equation,
\begin{equation}
    \bm{Y}_{(1)}=\bm{U}\bm{X}_{(1)},
\end{equation}
where $\bm{Y}_{(1)} \in \mathbb{R}^{L \times JK}$ and $\bm{X}_{(1)} \in \mathbb{R}^{I \times JK}$ are the matricization form in the I-mode respectively, and $\bm{U} \in \mathbb{R}^{L \times I}$ is the random normal compression matrix.  By multiplying  $\mathcal{X}$ with $\bm{U}$, the size of I mode is reduced. Suppose $\mathcal{X}$ are not sparse, there exist $LI^{3}=25,000,000,000$ times  of floating point multiplication computations which is massive and heavy. 

Here, we propose to use sparse projection to reduce the massive computations of floating points. Accoring the previous research \cite{verySparseProjection}, replacing non-sparse random normal distribution with sparse random normal distribution still enjoys some constant properties in the sense of statics, like the inner product and distance. Thus, we propose to offload the non sparse random projection to the sparse projection.

Correspondingly, instead of generating normal compression matrix, we construct the sparse  projection matrix  $\bm{U} \in \mathbb{R}^{L \times I}$, where $L \ll I$, containing entries
\begin{equation}
    \bm{U}(l,i)=
    \begin{cases}
\sqrt{s}, &\text{with prob. $\frac{1}{2s}$},\\
0, &\text{with prob. $1-\frac{1}{s}$},\\
-\sqrt{s}, &\text{with prob. $\frac{1}{2s}$},\\
\end{cases}
\end{equation}
where $s=\frac{I}{L}$, i.e., the compression ratio along the I-mode. The entries within each row are mutual-independent while the entries across different rows are fully independent. Each row will contains $s$ nonzero elements in expectation with saving $(1-\frac{1}{s}) \times 100\%$  floating point computations. As previous research reported, the properties of statistic are preserved with $s$ maximum up to $\frac{I}{\log I}$. Taking the compression of the above tensor $\mathcal{Y} \in \mathbb{R}^{500 \times 500 \times 500}$ for example, sparse projection will save $60\%$ floating point computations. 

\subsubsection{Mixed  Precision Acceleration using Tensor Core}


Tensor cores are programmable matrix-multiply-and-accumulate units that can deliver up to 125 Tensor TFLOPS for computations. It provides a significant acceleration for the operation $\bm{D}=\bm{A}\bm{B}+\bm{C}$, where $\bm{A},\bm{B}$ and  $\bm{C}$ are FP16 matrices while the accumulation matrices $\bm{C}$ and $\bm{D}$ are FP32 matrices. Thus, we fully make use of the properties of Tensor cores to accelerate the compression stage. 

We convert $\bm{U}_{p}$, $\bm{V}_{p}$, $\bm{W}_{p}$ and tensor block $\mathcal{B}_{n}$ read in memory from FP32 to FP16, and the accumulated replica $\mathcal{Y}_{p}$ to FP32 to perform mixed precision acceleration using tensor cores.

However, there is a high rounding error for the precision conversion of  which cause  cumulative error for the accumulation of the replicas. Here, we propose to factorize FP32 format data to FP16 format data and    its residual error from conversion. Here is an example shown in  Fig. \ref{fig:precision conversion}.  A FP32 format data $x_{32}$ is first converted to FP 16 format data $x_{16}$ with residual error $e_{16}$. To avoid numerical underflow for $e_{16}$, an advanced computation is executed with scaling of exponent term to obtain $\hat{x}_{16}$. $x_{16}$ and its corresponding residual error $\hat{x}_{16}$  participate in the following  computations. 

We make a preliminary experiment for matrix-multiply-and-accumulate operation $\bm{D}=\bm{A}\bm{B}+\bm{C}$, where $\bm{D} \in \mathbb{R}^{M \times N}, \bm{A} \in \mathbb{R}^{M \times K}, \bm{B} \in \mathbb{R}^{K \times N}, \bm{C} \in \mathbb{R}^{M \times N}$, using mixed precision methods and the results are shown in Fig. \ref{fig:precision conversion time } and Fig. \ref{fig:precision conversion error}. We denote \textit{FF} as float-float computation, \textit{HF} as half-float computation with no modification  and \textit{HFR} as half-float computation with modification using residual error. The MSE is the mean squared error of \textit{HF} or \textit{HFR} respect to \textit{FF}. It can be shown that compared with \textit{HF}, \textit{HFR} enjoys a significant improvement for computation precision with a relative small lost for speed.




The compression process can be factorize as following, 
\begin{equation}
    \label{residual error compression}
    \begin{split}
    \bm{y}_{p}=&({(\bm{U}_{p}}+\hat{\bm{U}}_{p})\otimes{(\bm{V}_{p}+\hat{\bm{V}}_{p})}\otimes{(\bm{W}_{p}+\hat{\bm{W}}_{p})})\textbf{Vec}(\mathcal{X}+\hat{\mathcal{X}})\\
    \approx &(\bm{U}\otimes\bm{V}\otimes\bm{W})\textbf{Vec}(\mathcal{X})+(\hat{\bm{U}}\otimes\bm{V}\otimes\bm{W})\textbf{Vec}(\mathcal{X})+\\
    &(\bm{U}\otimes\hat{\bm{V}}\otimes\bm{W})\textbf{Vec}(\mathcal{X})+(\bm{U}\otimes\bm{V}\otimes\hat{\bm{W}})\textbf{Vec}(\mathcal{X})+\\
    &(\bm{U}\otimes\bm{V}\otimes\bm{W})\textbf{Vec}(\hat{\mathcal{X}}),
\end{split}
\end{equation}
where $\bm{U}_{p},\bm{V}_{p},\bm{W}_{p},\mathcal{X}$ are stored in FP16 format, $\hat{\bm{U}}_{p},\hat{\bm{V}}_{p},\hat{\bm{W}}_{p},\hat{\mathcal{X}}$ are the residual error for the precision  conversion from FP32 to FP16 and we only consider the computations with first-order residual error and ignore the computations for the high-order residual error.

%where $\mathcal{\hat{X}}$ is the FP16 format and $\mathcal{\hat{X}}_{e}$ is the rounding error for conversion, i.e., $\mathcal{\hat{X}}_{e}=\mathcal{X}-\mathcal{\hat{X}}$. Then, we respectively calculate the compression replicas with $\mathcal{\hat{X}}$ and $\mathcal{\hat{X}}_{e}$ and merge to the same replica. 
 
%\begin{equation}
%    \label{compress equal matrix}\begin{split}
%    \bm{y}_{p}&=\textbf{Vec}(\mathcal{Y}_{p})\\
%    &=({\bm{U}_{p}}\otimes{\bm{V}_{p}}\otimes{\bm{W}_{p}})(\textbf{Vec}(\mathcal{X}))\\
%    &=((\bm{U}_{p}\bm{A})\odot(\bm{V}_{p}\bm{B})\odot(\bm{W}_{p}\bm{C})),
%\end{split}
%\end{equation}
 
%There is a high gap between the speed for processing floating points with single precision and the double precision for GPUs. Taking TITAN RTX as example, the theoretical performance  for floating point computation with double precision (FP64) is $509.8$ GFLOPS while that with single precision (FP32) is only up to $16.31$ TFLOPS which is slower maximum up to $31.34 \times$ . Despite of the high performance for single precision, the storage and computation with double precision enjoy a more stable and accurate result. Thus, We exploit mixed precision strategy to made a trade-off between precision and speed. 

%We convert $\bm{U}_{p}$, $\bm{V}_{p}$, $\bm{W}_{p}$ and tensor block $\mathcal{B}_{n}$ to single precision format before compressing the tensor block because compression is the time bottleneck of this stage. Once we get the replica $\mathcal{Y}_{p}^{n}$ after compression, we convert it from single precision to double precision when adding it to $\mathcal{Y}_{p}$, for addition is not time consuming at this stage, to avoid further loss of accuracy. In this way, we get about  10x speedup at compression stage while the loss is still in acceptable range. 




%For the baseline, the scheme compress each mode of tensor by Gaussian random matrices which contains massive floating point  computations. According  to some researches in analysis of big data, the Gaussian random projection can be replaced by sparse projection with a proper scale ratio, which is maximum up to $\log D$ where $D$ is the dimension of the initial data, and still enjoy a tolerant accuracy in the sense of statistics. Thus we propose to generate the  mode  compression matrices drawn from a given distribution $\{-1,0,1\}$ with a given probability $\{\frac{1}{2s},1-\frac{1}{s},\frac{1}{2s}\}$, where the compression ration is maximum up to $\frac{D}{\log D}$.

% A respective high compression ratio guarantees a sufficient sparsity in the compression mode matrices. Thus we organize the sparse compression mode matrices in CSR format and utilize the sparse matrix to matrix multiplication routine 
% in cuSparse library to reduce the massive time consuming floating point computations.





\subsubsection{Improving the  GPU Utilization}

 In regular GPU implementation, the matrix multiplications  for all blocks and all replicas are computed one by one on GPU.  However, the preliminary experiment result showed that the vanilla program did not fully utilize the resources of of GPUs.

We improve the utilization of GPUs by exploiting gemmBatched routine in cuBLAS libraries to run batch matrix multiplications in parallel on GPU. Due to the independence of all  compression replicas from one same block, we organize and compute the multiple matrix multiplications in  batches, accumulate and obtain the compression replicas in parallel. The batched scheme is illustrated in Fig. \ref{batched-schemes}.  The block tensor $\mathcal{B}_{n}$ is read from memory and respectively compressed by the batch organized ${\{\bm{U}^{n}_{p}\}}_{p=1}^{P}$, ${\{\bm{V}^{n}_{p}\}}_{p=1}^{P}$ and ${\{\bm{W}^{n}_{p}\}}_{p=1}^{P}$ to obtain the sub-relicas ${\{\mathcal{Y}^{n}_{p}\}}_{p=1}^{P}$ which will be accumulated to  ${\{\mathcal{Y}_{p}\}}_{p=1}^{P}$, where  ${\{\bm{U}^{n}_{p}\}}_{p=1}^{P}$, ${\{\bm{V}^{n}_{p}\}}_{p=1}^{P}$ and ${\{\bm{W}^{n}_{p}\}}_{p=1}^{P}$ are the components for compressing $\mathcal{B}_{n}$. 

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.20]{Figures/gemmbathced.png}
    \caption{Illustration of the batched matrix multiplication on compression stage. The  $\bm{U}^{n}_{p}, \bm{V}^{n}_{p}$ and $\bm{W}^{n}_{p}$ are organized in batches and parallely compress the block $\mathcal{B}_{n}$ to obtain $\mathcal{Y}^{n}_{p}$, $p=1,2,..., P$. }
    \label{batched-schemes}
\end{figure}


\subsection{Optimization Factorization Stage}
Our \textit{trillion-tensor} scheme mainly differs on the factorization stage between the dense and sparse conditions. For the dense condition, we permute all the factorization mode matrices of the compression replicas to a common scaling and permutations, solve a master linear square problem and obtain the the mode matrices after recovering the scaling and permutations. While for sparse condition, after factorizing the only replica into the mode matrices, we directly exploit the latent sparsity to solve the sparsity or error constraint  linear  problem using OMP-Cholesky algorithm. 


Factorization stage mainly consists of CP decomposition and solving linear square problems for factorization matrices of mode matrices. CP decomposition plays an important role in factorization stage.   Error constraint optimization from line $2$ to $13$ comprises of lots of times of solving least square problem. Thus, there remains a challenge that how to efficiently solve the linear square problems on the factorization stage. Here, we carefully design and implement the efficient strategy according to the facing situations.









%\section{Sparse Tensor and Multi-GPU Implementations}
 
% Multi-GPU 是技巧
 
%In this section, we will introduce our strategies for sparse tensor decomposition in \textit{exascale-tensor} scheme and show the implementations of multi GPUs.

%\subsection{Sparse Exascale-Tensor Decomposition}

%\begin{algorithm}[t] 
%\caption{Our Trillion-Tensor Scheme for Sparse Tensors} 
%\label{alg:Framworkforsparse} 
%\begin{algorithmic}[1] %这个1 表示每一行都显示数字
%\REQUIRE ~~\\ %算法的输入参数：Input
%tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$ with rank R; size of compression replicas, %$L, M, N$; 
%\ENSURE %算法的输出：Output
%mode matrices $(\bm{A}, \bm{B}, \bm{C})$;\\
%\STATE Randomly generate matrices $\bm{U}\in\mathbb{R}^{L \times I},\bm{V}\in\mathbb{R}^{M \times %J},\bm{W}\in\mathbb{R}^{N \times K}$,
%\label{ code:fram:compression }%对此行的标记，方便在文中引用算法的某个步骤
%%\FOR{$p=1$ to $P$}
%\STATE $\mathcal{Y} \gets$ compress $\mathcal{X}$ using $(\bm{U},\bm{V},\bm{W})$,
%\ENDFOR
%\label{code:fram:factorization}
%\label{code:fram:join}
%\STATE $(\bm{A}^{'},\bm{B}^{'},\bm{C}^{'})$ $\gets$ rank-R CP decomposition of $\mathcal{Y}$ via Alg. %\ref{alg:baseline CP},
%\STATE $\bm{A} \gets $ use OMP algorithm to solve for the $L_{1}$ constraint minimization problem %$\bm{A}^{'} = \bm{U}^{T}\bm{A}$, and likewise for $\bm{B}$ and $\bm{C}$, 
%\RETURN $(\bm{A}, \bm{B}, \bm{C})$. %算法的返回值
%\end{algorithmic}
%\end{algorithm}




%For the sparse tensors, the $\textit{exascale-tensor}$ scheme mainly consists of two stages, namely the compression stage same as that in the $\textit{exascale-tensor}$ scheme for dense tensors but here only one replica being created, i.e. $P=1$, and factorization stage is composed of CP decomposition of replica  and recovery of factorization matrices for raw data. 

%The difference for  sparse tensor decomposition in \textit{exascale-tensor} mainly in the factorization stage. To solve $\bm{A}=\mathop{\arg\min}_{\bm{A}} {\Vert \bm{A'}-\bm{U}\bm{A} \Vert}_{2}$ and likewise for $\bm{B}$ and $\bm{C}$, where ($\bm{A'},\bm{B'},\bm{C'}$) is the factorization matrix of the replica, different from the solving a least square problem for dense tensor decomposition, here, we fully utilize the sparsity of the raw tensor and its factorization matrix, view the $L_{2}$ minimization problem as a $L_{1}$ constraint minimization problem $\bm{A}=\mathop{\arg\min}_{\bm{A}} {\Vert \bm{A'}-\bm{U}\bm{A} \Vert}_{1}$. Here, we exploit  OMP-Cholesky  algorithm to solve the sparse-constraint least square problem to obtain $\bm{A}$ and likewise for $\bm{B}$ and $\bm{C}$.  

%The pseudocode for sparse tensor decomposition is shown in Alg. \ref{alg:Framworkforsparse}. From line $1$ -- $2$, the raw data $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$ is compressed into one replica $\mathcal{Y} \in \mathbb{R}^{L \times M \times N}$.  We use ALS to optimize  CP decomposition in Line $3$ and we utilize error-constraint OMP-Cholesky algorithm. 



%\subsection{Handing More Large Scale Sparse Tensors}

%Compared with the trillion-tensor scheme for dense condition, the scheme for sparse condition enjoys a much more efficiency due to the reduced cost of the compressed replicas, but it can not afford a arbitrary high compression rate which depends on the properties of the compression sense algorithm used. Thus,  to handle the large scale sparse tensors in our trillion-tensor scheme for sparse conditions, the bottleneck falls on the factorization of the compression replicas which might exceeds the maximum computation capacity of the CP decomposition. Here, we propose the embedded $\textit{Twice-Compression}$ method to combine the solutions for dense condition with sparse condition to handle more large scale sparse tensors with less efficiency loss. 

%Consider a large scale sparse tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$, for sparse condition, we compress it into the relative small tensor $\mathcal{Y} \in \mathbb{R}^{L \times M \times N}$ but it still exceeds the maximum computation capacity of CP decomposition. Note that the compression replica $\mathcal{Y}$ is usually dense, so we can exploit the trillion-tensor scheme for dense condition to run the tensor decomposition and obtain the factorization mode matrices of the compression replica. Then, we exploit the OMP algorithm to further recover the factorization mode matrices of the large scale tensor from the compression space.  

%Due to the property of the kronecker product, we have 
%\begin{equation}
%\label{compress twice process}\begin{split}
%    \bm{y}&=\textbf{Vec}(\mathcal{Y})\\
%    &=({\bm{U}_{p}}\otimes{\bm{V}_{p}}\otimes{\bm{W}_{p}})((\bm{U}\bm{A})\odot(\bm{V}\bm{B})\odot(\bm%{W}\bm{C}))\\
%    &=(({\bm{U}_{p}}\bm{U}\bm{A})\odot({\bm{V}_{p}}\bm{V}\bm{B})\odot({\bm{W}_{p}}\bm{W}\bm{C}))\\
%    &=(\hat{\bm{U}_{p}}\bm{A})\odot(\hat{\bm{V}_{p}}\bm{B})\odot(\hat{\bm{W}_{p}}\bm{C}),
%\end{split}
%\end{equation}
%where $\bm{U}_{p}$ is the random mode matrix for the first compression stage while $\hat{\bm{U}}$ is for the second compression stage, likewise for $(\bm{V}_{p},\hat{\bm{V}})$ and $(\bm{W}_{p},\hat{\bm{W}})$. Thus, the second time of  the compression stage is implicit that we can pre-process the random mode matrices by multiplying the corresponding random compression matrices of two stages with each other.


%Exploiting the feature that the compression replica at the begginning of  the implicit , the embedded $\textit{Twice-Compression}$ method for sparse condition actually obtain an extra compression rate income.  Compared with directly exploiting the scheme for dense condition, it demands for much fewer compression replicas. Thus, the $\textit{Twice-Compression}$ method can address the trouble for the limitations of the CP decomposition with the compression replica,  achieve the more large scale  sparse tensor decomposition. The reduction for the size for compression replicas also speedup the factorization stage. A proper setting of the compression rates for the twice compression can achieve the balance of the high efficiency and large computation capacity.  


%\begin{algorithm}[t] 
%\caption{Embedded Twice-Compression Trillion-Tensor %Scheme} 
%\label{alg:Twice compression Framwork} 
%\begin{algorithmic}[1] %这个1 表示每一行都显示数字
%\REQUIRE ~~\\ %算法的输入参数：Input
%tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times %K}$ with rank F; dimensions of first compression %replicas, $L, M, N$;dimensions of second compression %replicas, $qL, qM, qN$; the number of replicas $P$; the %number of common columns $S$.
%\ENSURE %算法的输出：Output
%mode matrices $(\bm{A}, \bm{B}, \bm{C})$;\\
%%\STATE Randomly generate matrices $\bm{U}_{p} \in %\mathbb{R}^{qL \times L},\bm{V}_{p} \in \mathbb{R}^{qM %\times M},\bm{W}_{p} \in \mathbb{R}^{qN \times N}$, %$p=1,2, .., P$, and set the first $S$ columns the same, %and randomly generate matrices $\bm{U} \in \mathbb{R}^{L %\times I},\bm{V} \in \mathbb{R}^{M \times J},\bm{W} \in %\mathbb{R}^{N \times K}$,
%\label{ code:fram:compression %}%对此行的标记，方便在文中引用算法的某个步骤
%\FOR{$p=1$ to $P$}
%\STATE $\mathcal{Y}_{p} \gets$ compress $\mathcal{X}$ %using $(\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{V},\bm{W}_{p}\bm{%W})$ , for $p = 1, .., P$,
%\ENDFOR
%\label{code:fram:factorization}
%\STATE $(\bm{A}^{'},\bm{B}^{'},\bm{C}^{'})$ $\gets$ run %the decomposition stage of rank-F compressed based CP %decomposition of $\{\mathcal{Y}_{p}\},p=1,2,...,P$,
%\STATE $\bm{A} \gets $ use OMP algorithm to solve for %the $L_{1}$ constraint minimization problem $\bm{A}^{'} %= \bm{U}\bm{A}$, and likewise for $\bm{B}$ and $\bm{C}$,
%\label{code:fram:join}

%\RETURN $(\bm{A}, \bm{B}, \bm{C})$. %算法的返回值
%\end{algorithmic}
%\end{algorithm}

%For instance, to handle a large scale sparse tensor $\mathcal{X} \in \mathbb{R}^{6,000 \times 6,000 \times 6,000}$,  in our trillion-tensor scheme for dense tensor, we can compress the large scale tensor into a series of relative  small  compression replicas $\mathcal{Y}_{p} \in \mathbb{R}^{200 \times 200 \times 200},p=1,2,...,30$ for simplify computation which occupied the memory of $30\times 200 \times 200 \times 200$ elem data types. When exploiting the sparse scheme, there is one relative large scale  compression replica $\mathcal{Y} \in \mathbb{R}^{600 \times 600 \times 600}$ which occupied the memory of $600 \times 600 \times 600$ elem data types. For the embedded $\textit{Twice-Compression}$ method, we can set the implicit number of replicas, $P=3$, for the second compression stage. And we will have $3$ replicas $\mathcal{Y}_{p} \mathbb{R}^{200 \times 200 \times 200}$, $p=1,2,3$, need to be factorized. And the demand memory is $3 \times 200 \times 200 \times 200$ elem data types. The embedded $\textit{Twice-Compression}$ method costs memory  $9\times$ less than the direct method for sparse condition and $10\times$ less than the method for dense condition. Correspondingly, the smaller size  and fewer number of the compression replicas will further accelerate the algorithm compared with the direct method for sparse and dense conditions. 

%\subsection{Multi-GPU Trillion-Tensor Scheme}
%We design a multi-GPU scheme for exascale-scale CP tensor decomposition to fully utilize the multiple GPUs in the computing device. Benefit from the property of the tensor contraction and spliting strategy used in the compression stage, the compression of each tensor block is independent of each other. And for muli-replicas conditions in our algorithm, i.e. dense condition and more large scale spase condition, there are multiple replicas need to be factorized and the decomposition of each  replica is also independent of each other. Thus, we can distribute the computation among multiple GPUs to compute in parallel. Suppose there are $c$ GPUs, denoted as $GPU_{1}$, ..., $GPU_{c}$, in the given computing device and the size of tensor is $I \times J \times K$. We set the size of block read in RAM one time is $B_{1 \times B_{2} \times B_{3}}$ and the number of total blocks $N=\frac{I \times J \times K}{B_{1} \times B_{2} \times B_{3}}$. We perform the parallel computation as follows:

%\begin{itemize}
    %\item CPU calculates and prepares the offset address of each block, $Addr_{1}, ..., Addr_{N}$, %then distributes them to a series of sets $C_{1}, ..., C_{c}$ of which number is related to the %number of GPUs and lastly send the sets to corresponding GPUs. The number of Address of each set %$\vert C_{i} \vert$ is proportional to the performance  of the $GPU_{i}$, $i=1, ..., c$, and we %have $\sum\limits_{i=1}^{c}\vert C_{i} \vert = N$.     
%    
 %   \item $GPU_{i}$ receives the to-be-processed address set $C_{i}$, and sequentially compress the %block referenced by the given set. For multi-replica conditions, to maximize the utilization of GPU, %we exploited the batch matrix multiplication to compress the block to multiple blocks in parallel. %The process of reading block is asynchronous between different GPUs which means that only one GPU %can access the data at the same time. Upon completion, the direct GPU to GPU communication will be %launched to send the result of $GPU_{i}$ to $GPU_{1}$ to form the final result.
 %   
  %  \item The following steps depends on the number of replicas.
   % \begin{itemize}
    %    \item For one replica condition, $GPU_{1}$ factorize the compressed tensor and the recovery %stage will be launched to obtain the estimation of the  mode matrices.
     %   
      %  \item For multi-replica condition, $GPU_{1}$ will construct a series of set $C_{1}, ..., %C_{c}$ of which set contains a number of replicas. Likewise, $C_{i}$ is is proportional to the %performance  of the $GPU_{i}$, $i=1, ..., c$. $GPU_{1}$ distributes the sets to corresponding %GPU and each GPU independently factorizes the compressed replicas. Upon completion, the results %from all GPUs will be merged to $GPU_{1}$ and $GPU_{1}$ continue to carry out the following %recovery stage to obtain the estimated mode matrices. 
    %\end{itemize}
%\end{itemize}
%The scheme fully utilize the advantages of multiple GPUs and independence of key operations in the algorithm  to accelerate the overall computation. The  data, except the address sets, transfer from GPU to GPU and no intermediate variables transferred back to CPU for reducing communication cost. And the direct GPU to GPU communication can be implemented by the memory copying routine supplied by the pyCUDA library.

==> dac24/Sections/Introduction.tex <==
\section{Introduction}
%尚未修改
%1.background of large-scale tensor decomposition with two or three examples or applications.
%target issue 为什么处理大规模 为什么有这个需求 
%2.existing work has limitations
%3.target issue
%5.challenges
%6.what we do

Real-world big data are naturally modeled as a  multidimensional array, called a tensor. Examples include a time-evolving social network, knowledge base and web data. Tensor decomposition is the basis of many machine learning applications including graphic analysis, image classification, data mining, etc. CP tensor decomposition is one of major tensor decomposition algorithms. 
%talk about challenges


% 逻辑  罗列给出exascale的理由,让人知道exascle很重要,应用例子和技术的重要性,立题（体系结构角度）
In recent years, the size of tensors becomes increasingly large, approaching trillion ($10^{12}$)  to exascale (billion billion, $10^{18}$) of  nonzero elements. Due to the limitation of the main memory, CP  tensor decomposition algorithm is impractical for large-scale tensors. To address this problem, there have been proposed many adaptive methods for large-scale tensor decomposition, including CDTF \cite{fullyscaleble} and 2PCP  \cite{2PCP} for CP tensor decomposition. These methods may handle tensors with each mode up to millions. However, the input tensors are required to be extremely sparse, where the total number of nonzero elements is up to millions. On the other hand, the widely used tensor toolboxes Tensor Toolbox \cite{TTB_Software} and TensorLy \cite{tensorly} operate in the main memory, but cannot support large dense tensors, as shown in Table \ref{tab:results}. The PARACOMP (parallel randomly compressed cubes) algorithm \cite{paracomp} was a promising compression-based tensor decomposition algorithm, but the reported size was $500 \times 500\times 500$. 
%But we are convinced that the potential of this method should not be limited to this scale.%When the size in each mode of tensor decreases but the sparsity decreases, for example, a tensor with the size $10000 \times 10000 \times 10000$ and the number of nonzero elements close to $10^{12}$, existing methods are not applicable. A challenging problem which arises in this domain is extra large scale,  at the element level, tensor  decomposition. And the bottleneck of existing large-scale dense tensor decomposition algorithm is the limitation of main memory,  for which the full tensor can not be loaded in memory. 

\begin{table}[t]
\centering
\small
\caption{Comparison of supported tensor sizes.  Our proposed Exascale-Tensor supports
$58,000 \times$ larger tensors.}\label{tab:results}
\begin{tabular}{ccc}
\toprule
Work & Tensor Size\\
\midrule
TensorLy \cite{tensorly}& $800 \times 800 \times 800$\\
Tensor Toolbox \cite{TTB_Software} & $1,200 \times 1,200 \times 1,200$\\
PARACOMP \cite{paracomp}& $500 \times 500 \times 500$\\
Exascale-Tensor (\textbf{Ours}) & $1,000,000 \times 1,000,000 \times 1,000,000$\\
\bottomrule
\end{tabular}
\end{table}

There are three primary challenges with exascale-scale tensor decomposition. $1)$ Designing a compression method to process an ``out-of-memory" tensor; 
$2)$ Exploring an appropriate trick to recover the permutations and scaling of the full mode factorization matrices;  
And $3)$ implementing efficient parallel schemes both on CPUs and GPUs, respectively.

%In this paper, we implement a compression-based algorithm \textit{trillion-tensor} for trillion-scale (number of elements) CP tensor decomposition by trading computation for storage.  We make full use of the parallelism of tensor operations to accelerate the proposed trillion-tensor scheme on CPUs and GPUs, respectively. In our experiments, we test tensors ranging from million-scale to trillion-scale and obtain a relatively low mean squared error.  Comparing to the baseline method PARACOMP, trillion-tensor supports $8,000$ larger tensors and a speedup up to $6.95\times$.  


In this paper, we explore the potential of a compression-based algorithm and implement $\textit{trillion-tensor}$ to support exascale-scale (number of elements) CP tensor decomposition by trading computation for storage. First, we  implement a baseline version CPU-based exascale-tensor scheme for sparse tensors and dense tensors, respectively. Second, we design and implement a baseline GPU-based exascale-tensor scheme and propose techniques to optimize memory accesses, GPU utilization and communications. Third, we propose techniques to optimize the compression stage and decomposition stage and handle more large scale tensors. We also carefully design a high performance exascale-tensor scheme on multiple GPUs. In our experiments, we test tensors ranging from million-scale to exascale-scale and obtain a relatively low mean squared error. Evaluation results show that $\textit{trillion-tensor}$  supports $8,000$ larger tensors and a speedup up to $6.95\times$, compared with the baseline method PARACOMP \cite{paracomp}.


The remainder of this paper is organized as follows.
In Section 2, we describe notations and introduce the CP tensor decomposition algorithm. Section 3 describes the proposed compression-based algorithm \textit{exascale-tensor} and the parallel acceleration analysis. In Section 4, we presents the design, implementation and optimization of the proposed high-performance \textit{exascale-tensor} scheme. In Section 5, we present performance evaluations on the reconstruction error and time consumption. In Section 6, we conclude this paper. 
%In this paper, we implement the compression-based algorithm \textit{trillion-tensor} to achieve the trillion-scale, at element level, CP tensor decomposition by trading computation for storage.  Furthermore,  we  make  full  use  of  the  parallelism of tensor operations to accelerate the proposed scheme  on  CPUs  and  GPUs,  respectively.   In our experiments, we test tensors ranging from million-scale to trillion-scale and obtain a relatively  low  mean  squared  error.  Comparing to the baseline method, trillion-tensor supports 8,000 larger tensors and a maximum of $6.95\times$ speedup.

%In this paper,  we exploit the potential of the compression-based algorithm. In our work, we exploit the computation cost to exchange for the storage consumption, applying the compression-based algorithm to pursue trillion-scale CP tensor decomposition. And resort to the uniqueness of CP decomposition, we proposed a solution to recover the factorization mode matrices from  the permutations and scaling.  Furthermore, to reduce the time consumption as much as possible, we develop two different parallel frameworks on the CPUs and GPUs respectively to make a preliminary acceleration. 


%Previous work \cite{paracomp} proposed a compression-based tensor decomposition algorithm which compresses the tensor to small replicas and get the factorization mode matrices from the independent CP decomposition results of compression replicas. In our work, we further exploit its potentialities for extra large-scale tensor decomposition and make preliminary acceleration to reduce the huge time consuming on one PC.










==> dac24/Sections/Large-scale_CP_Tensor_Decomposition.tex <==
\section{CP Tensor Decomposition}
\label{tensor_decompositon}

%For details about tensor decomposition, please refer to \cite{tutorials}. 
%Due to space limitations, here we only briefly summarize key concepts and operations related to our work.

\textbf{Notations}:
 We use uppercase calligraphic letters to denote third-order tensors, e.g.,  $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$, uppercase boldface letters to denote  matrices and lowercase boldface letters to denote vectors, e.g., $\bm{A} \in \mathbb{R}^{I \times J}$ and $\bm{a} \in \mathbb{R}^{I}$. $\bm{X}_{(n)}$ denotes the $n$-mode matricization of a tensor $\mathcal{X}$. We use $\odot$ to denote Khatri-Rao product and $\otimes$ to denote the tensor (Kronecker) product, which correponds to the outer product for vectors.
%For tensor $\mathcal {X} \in \mathbb{R}^{I \times J \times K}$, the $(i, j, \ell)$-th entry is $\mathcal{X}_{i, j, \ell}$.We also use $\mathcal{X}(:,:,\ell),\mathcal{X}(:,j,:) and \mathcal{X}(i,:,:)$ to denote the frontal,lateral,horizontal slices that are matrices.Likewise, $\bm{A}(i,:)(\bm{A}(:,j))$ denotes the i-th row of the matrix $\bm{A}$(respectively,j-th col).%
 



\subsection{CP Tensor Decomposition  Algorithm}
\begin{algorithm}[t] 
\caption{ALS algorithm for CP tensor decomposition} 
\label{alg:baseline CP} 
\begin{algorithmic}[1] %这个1 表示每一行都显示数字
\REQUIRE a third-order tensor $\mathcal{X}$ of size $I \times J \times K$, rank $R$, and maximum number of iterations $T$,
\ENSURE %算法的输出：Output
matrices $(\bm{A}, \bm{B}, \bm{C})$.\\
\STATE Initialize $\bm{A} \in \mathbb{R}^{I \times R}, \bm{B} \in\mathbb{R}^{J \times R}, \bm{C} \in \mathbb{R}^{K \times R}$, $t=0$,
\WHILE{$t \leq T$ and NOT converged}
    \STATE $\bm{A} \gets  \bm{X}_{(1)}(\bm{C}\odot\bm{B})(\bm{C}\bm{C}^{T}*\bm{B}\bm{B}^{T})$，
    \STATE $\bm{B} \gets \bm{X}_{(2)}(\bm{C}\odot\bm{A})(\bm{C}\bm{C}^{T}*\bm{A}\bm{A}^{T})$，
    \STATE $\bm{C} \gets  \bm{X}_{(3)}(\bm{B}\odot\bm{A})(\bm{B}\bm{B}^{T}*\bm{A}\bm{A}^{T})$，
\ENDWHILE
\RETURN $(\bm{A}, \bm{B}, \bm{C})$. %算法的返回值
\end{algorithmic}
\end{algorithm}

For a data tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$, the CANDECOMP/PARAFAC (CP) tensor decomposition represents it as a linear combination:
\begin{equation}
\label{cp_equation}
    \mathcal{X} = \sum\limit_{r=1}^{R}\bm{a}_{r}\otimes\bm{b}_{r}\otimes\bm{c}_{r}, 
\end{equation}
where $\bm{a}_{r} \in \mathbb{R}^{I}, \bm{b}_{r} \in \mathbb{R}^{J}$, $\bm{c}_{r} \in \mathbb{R}^{K}$. The CP tensor decomposition in  (\ref{cp_equation}) can be written in a matrix form
\begin{equation}
\begin{split}
    &\bm{X_{(1)}}\approx\bm{A}(\bm{C}\odot\bm{B})^{T},\\ &\bm{X_{(2)}}\approx\bm{B}(\bm{C}\odot\bm{A})^{T},\\ &\bm{X_{(3)}}\approx\bm{C}(\bm{B}\odot\bm{A})^{T},
\end{split}
\label{cp_lst_equation}
\end{equation}
where $\bm{A} \in \mathbb{R}^{I \times R}$, $\bm{B} \in \mathbb{R}^{J \times R}$, $\bm{C} \in \mathbb{R}^{K \times R}$ have the corresponding columns ${\{\bm{a}_{r}\}}_{r=1}^{R}$, ${\{\bm{b}_{r}\}}_{r=1}^{R}$ and ${\{\bm{c}_{r}\}}_{r=1}^{R}$,  respectively.  

%\yanglet{Relate (2) to lines 3-5 in Alg. 1}

The alternative least squares (ALS) algorithm is widely used to obtain the mode matrices $(\bm{A}, \bm{B}, \bm{C})$, as given in Alg. \ref{alg:baseline CP}. First, ($\bm{A},\bm{B},\bm{C}$) are randomly initialized in line $1$, e.g., following an identical independent normal distribution. Then, the while-loop in line $2$--$6$ alternatively fixes two matrices and solve the least square problems, as shown in Eq. (\ref{cp_lst_equation}), to obtain the third matrix. The whole-loop stops until the reconstruction error is below a preset threshold or the maximum number of iterations is reached.  

However, the above updates of $\bm{A}$, $\bm{B}$ and $\bm{C}$ require to load the full tensor $\mathcal{X}$ into the main memory. Thus, the capacity of  main memory becomes the bottleneck, restricting the supported tensor size. 


%\yanglet{Bottleneck or constraints.}

%\yanglet{What makes it challenging?}


\subsection{Motivation for Exascale Tensor Decomposition}
\label{compression_based_demo}
%基于前期工作（trillion), 进一步拓展到exascale； 解决一些挑战。

\yanglet{Relating Alg. 1 and combining Trillion-tensor, please motivate our task of exascale.}

The full tensor need to be loaded in main memory for solving the least square problems for line 3--6 in Alg. \ref{alg:baseline CP} which restricts its large scale applications with limited main memory. \textit{Trillion-Tensor} \cite{trillionCP} exploit compression-based algorithm  to tackle the restriction introduced by limited main memory for CP decomposition and  pursue the trillion scale tensor decomposition. \textit{Trillion-Tensor} mainly consists of three stags, compression state,  factorization stage  and recovering the scaling and permutations stage.  
 

Consider a rank-$1$ tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$ which can be decomposed to 3 vectors $\bm{a}$, $\bm{b}$, $\bm{c}$. Instead of decomposing tensor $\mathcal{X}$ directly, the   \textit{Trillion-Tensor}  algorithm for $\mathcal{X}$ consists of the following three steps:
\begin{enumerate}
    \item  Compression of $\mathcal{X}$: The input tensor $\mathcal{X}$ is  multiplied every slab from each axis respectively with random matrices $\bm{U} \in \mathbb{R}^{L \times I}$, $\bm{V} \in \mathbb{R}^{M \times J}$ and $\bm{W} \in \mathbb{R}^{N \times K}$ and  is compressed into reduced replica $\mathcal{Y} \in \mathbb{R}^{L \times M \times N}$.
    \item  Factorization of replicas $\mathcal{Y}$: using rank-1 CP decomposition, $\mathcal{Y}$ will be  factorized to 3 vectors $\hat{\bm{a}} \in \mathbb{R}^{I}, \hat{\bm{b}} \in \mathbb{R}^{J}, \hat{\bm{c}} \in \mathbb{R}^{K}$.
    \item  Recovery of factorization matrices ($\hat{\bm{a}},\hat{\bm{b}},\hat{\bm{c}}$): a least square problem  per mode will be solved to obtain factorization matrices of raw data, i.e. $\bm{a}=\mathop{\arg\min}_{\bm{a}} {\Vert \hat{\bm{a}}-\bm{U}\bm{a} \Vert}_{2}$,$\bm{b}=\mathop{\arg\min}_{\bm{b}} {\Vert \hat{\bm{b}}-\bm{V}\bm{b} \Vert}_{2}$ and $\bm{c}=\mathop{\arg\min}_{\bm{c}} {\Vert \hat{\bm{c}}-\bm{W}\bm{c} \Vert}_{2}$.
\end{enumerate}
%这个算法在应用大规模时存在怎样的挑战
The ALS algorithm  is utilized for CP decomposition in the second step.  

There remain two main  challenges when applied to large scale tensor decomposition. First, to factorize a large scale tensor, high compression ratio comes with more compression replicas to guarantee the stability of numerical calculation, and correspondingly more times of matrix multiplications on compression stage and CP decomposition on factorization stage, which introduce massive time consumption. Second, the storage for compression replicas is also considerable and largely restrict the maximum size of tensors that \textit{Trillion-Tensor} can handle. 


Note that there is no assumption of sparsity for the tensor in \texit{Trillion-Tensor}, and the storage for the compression replicas restricts the  application for larger scale. Thus, to achieve larger scale tensor decomposition, we make an assumption that the tensor is sparse. Exploiting the sparsity of tensors, we make an improvement on  \textit{Trillion-Tensor}, by compressing the large scale tensor twice, further reduce the memory storage for compression replicas to get over the bottleneck to support exascale tensor. The following sections will show the design  for \textit{Exascale-Tensor Decomposition}. 

%There remain challenges that how to compress the large scale tensors which are difficult to load in RAM for following factorization stage. For example, a tensor $\mathcal{T} \in \mathbb{R}^{3000 \times 3000 \times 3000}$ of double-precision floating-point format needs at least $200$GB space to store which is obviously unable to be loaded in RAM to be compressed. However, tensors much larger than $\mathcal{T}$ are really common. Furthermore, the compression stage and factorization stage comprise of lots of  times matrix multiplication and solving for least square problems which are both of high computation complexity. How to achieve more large scale CP tensor decomposition and how to finish the task in an bearable  limited time with limited devices but has relative high precision remains challenging. Efficient methods need to be proposed to reduce the heavy time consumption. 

%Suppose the server has a main memory of $125$ GB, for a given third-order tensor $\mathcal{X} \in \mathbb{R}^{I \times I \times I}$ with rank $F=0.1 I$, we compress $\mathcal{X}$ into relative small tensors $\mathcal{Y}_{p} \in \mathbb{R}^{L \times L \times L}$, $p=1,2,...,P$,  where  we roughly denote $L \ge F$ and  $P=\frac{L}{I}$. We have a  estimation of the maximum size of tensors which can be processed using \textit{Trillion-Tensor}  where $I=11,000$ i.e., the number of elements  in tensor is trillion scale. It should be noted that there is no assumption of dense or sparse for $\mathcal{X}$.   The assumption of sparsity has  a promotion influence in many research areas like the generalization of models in machine learning and high performance computations. Here, we can  exploit the power of sparsity to  further improve the performance of the scheme. We can use the compression sensing theory to simplify the compress stage in \textit{Trillion-Tensor} and utilize multiple times for compression to improve the compression ratio at the cost of number of replicas and loss of estimation increasing. The sparsity reduce the both  the overhead for storage and cost for computations. In this work, we design and optimize compression-based algorithm, and  achieve exascale tensor decomposition.




% \subsection{Supporting Exascale Tensors}


%Here, we roughly estimate the maximum size of tensors that can be compressed in our exascale-Tensor scheme. To simplify, we next assume ${I=J=K}$, ${L=M=N}$ and omit the storage capacity  of  temporary variables. Note that, in this process, variables that we at most have to store in the memory at the same time are as following(use BS to represent the size of the block):
%\begin{itemize}
    %\item one tensor block with size ${{BS} \times BS \times {BS}}$
    %\item $3$ mode  compression matrices $\bm{U} \in \mathbb{R}^{{BS} \times L}$, $\bm{V} \in %\mathbb{R}^{{BS} \times M}$ and $\bm{W} \in \mathbb{R}^{{BS} \times N}$
    %\item $P$ replicas already obtained, each replica with size ${L \times M \times N}$
    %\item one new replica, with size ${L \times M \times N}$
%\end{itemize} 
% Here, we roughly estimate the maximum size of tensors that can be compressed in our exascale-Tensor scheme. To simplify, we next assume ${I=J=K}$, ${L=M=N}$ and omit the storage capacity  of the random compression matrices and temporary variables. Note that, in this process, variables that we at most have to store in the memory at the same time are as following(use BS to represent the size of the block):
%\begin{itemize}
%    \item one tensor block with size ${{BS} \times BS \times {BS}}$
%    \item $3$ mode matrices $\bm{U} \in \mathbb{R}^{{BS} \times L}$, $\bm{V} \in \mathbb{R}^{{BS} \times M}$ and $\bm{W} \in \mathbb{R}^{{BS} \times N}$
%   \item $P$ replicas already obtained, each replica with size ${L \times M \times N}$
%    \item one new replica, with size ${L \times M \times N}$
%\end{itemize} 
%Now consider a server with $V=125$ GB main memory and infinity storage capacity which supports large enough size of tensors to store. 
%Therefore, with $L=M=N$, we have
%\begin{equation}
%\label{tensor_size_equation}
    %8({BS}^{3} + 3{BS} \times {L} + ({P+1}){L}^{3})\le125\times 1024^3
%\end{equation}
%And we will discuss the size of tensor $\mathcal{T} \in \mathbb{R}^{I \times I \times I}$ , stored in double format, under two different conditions.



 % Suppose the tensor $\mathcal{T} \in \mathbb{R}^{I \times I \times I}$ with rank $F=0.1 I$ is stored in double format and the server with $125$ GB main memory can handle $N_{e}=16777216000$ double numbers. For simplification,  to decompose the maximum size of tensor as much as possible,  we adopt an aggressive compression rate $\alpha=F$ to make sure the uniqueness  of CP decomposition with $\alpha$ compression replicas, i.e., each dimension to be compressed $\alpha$ times as $L=\frac{I}{\alpha}$, and omit the storage capacity  of the random compression matrices and temporary variables. Thus we have the strict $P\frac{I^3}{L^3} =\le N_{e}$. 
 
 %Under normal condition, the rank of tensor $\mathcal{T}$ is $F=0.1 I$ . In order to decompose the maximum size of tensor as much as possible,  we adopt an aggressive compression rate ${P}=\frac{I}{F}$ to make sure the uniqueness of CP decomposition with ${P}$ compression replicas, i.e., each dimension to be compressed ${P}$ times as $L=\frac{I}{P}$. When {BS}=1000, substitute {P}=10, and {L} = ${\frac{I}{P}}$ = {0.1I} into Equation (4), we can obtain {I} is about {11, 000}. This means the largest tensor we can deal with under this usual condition is with size ${11, 000 \times 11, 000 \times 11, 000}$.

%On the other hand, if the rank of the tensor is extremely low, like {5} or {10}, we can set {L=15}. When {BS}=1000, substitute {L} = {15} and {P} = ${\frac{I}{L}}$ into Equation (4), we can obtain {I} is about {70, 000, 000}. This means the largest tensor we can deal with under the low rank condition is with size ${70, 000, 000 \times 70, 000, 000 \times 70, 000, 000}$. However, we have to deal with about {4, 600, 000} replicas.

%Furthermore, if the tensor is sparse, we can use the compression sensing theory to  calculate just one replica and recover the mode matrices which reduce the storage for the compression replica largely. And the use of mixed precision and sparse projection which are included in later subsections make the size of tensor larger. 
 
 %And we can exploit twice or more times compression method to pursue the extra large scale tensor decomposition. For example, to decompose a sparse extra-scale tensor with extra low rank, say $\mathcal{X} \in \mathbb{R}^{1, 000, 000 \times 1, 000, 000 \times 1, 000, 000}$ with rank $5$, decomposition, we can first use the sparse projection with a relatively aggressive compression rate $\sqrt{D}=1, 000$ where $D=1, 000, 000$ is the size of the extra tensor in one mode and get a relatively small dense tensor $\mathcal{T} \in \mathbb{R}^{1,000 \times 1,000 \times 1000}$. Then we compress $\mathcal{T}$ to $10$ replicas $\mathcal{Y}_{p} \in \mathbb{R}^{100 \times 100 \times 100}$, $p=1, 2, ..., 10$, and then use the replicas to obtain the factor matrices of $\mathcal{T}$, and then we use the compression sensing algorithm to recover the factored matrices of the initial extra scale tensor $\mathcal{X}$. The main memory needed for this condition is only around $1$ GB.

%PARACOMP (parallel randomly compressed cubes) \cite{paracomp} is a compression-based algorithm that has the potential to support large tensor decomposition. It first uses a set of random matrices to compress the tensor $\mathcal{X}$ into reduced-size replicas ${\{\mathcal{Y}_{p}\}}_{p=1,2,...,P}$, then each replica $\mathcal{Y}_{p}$ will be independently factored into mode matrices $\{(\bm{A}_{p}, \bm{B}_{p}, \bm{C}_{p})\}_{p=1,2,...,P}$. After proper permutation and scaling, solving a master linear squares problem per mode will result in the full mode loading matrices $(\bm{A}^{*}, \bm{B}^{*}, \bm{C}^{*})$.

%Multi-Way Compressed Sensing for Sparse Low-Rank Tensors %\cite{comp2012} proved the 
%correctness to apply the compressed sensing theory into the decomposition of  third-order sparse tensors and suggested a two-step process: fitting the low-rank model into the compressed domain, and exploiting the CP decomposition and sparsity constrained algorithms to restore the mode matrices of tensors in uncompressed space.







==> dac24/Sections/Performance_Evaluation.tex <==
\section{Performance Evaluations}

% Evaluate one Stage


In this section, we will provide numerical experiment results to show the  performance of our work on various scales of tensors from one hundred million scale to exascale.

\subsection{Experimental Settings}

We conduct our experiments on a server which has two Intel(R) Xeon(R) Gold 5118 CPUs. Each of CPUs has 12 cores @2.30GHz supporting 24 hardware threads. There is a Titan RTX GPU which consists of 24 GB device memory. There are 256 GB DDR4 memories on the server. We show the mean squared error (MSE) to measure the accuracy and speedups of baseline versus optimization schemes. The speedups is defined as  (\textit{baseline running time})/(\textit{optimized running time}).


In our experiment, we will show the results of our algorithm on dense tensor, sparse tensor and exascale sparse tensor. The factorization of the dense tensor, i.e., with no assumption of sparsity and not using compressive sensing method, is one of the important step of \textit{Exascale-Tensor} algorithm.   The factorization of the the sparse tensor directly uses the sparsity of tensors and exploits  compression sensing method to obtain the full mode matrices of large scale tensors. \textit{Exascale-Tensor} makes full use of the sparsity of tensors with compression sensing theory and exploits the factorization for dense tensor with 2-stage compression  to decompose exascale tensors. 

For the evaluation of factorization for dense tensors, we test cases on scales ranging from one hundred million to one trillion which approaches the limitations restricted by the device. For each case, we first generate the mode matrices $\mathit{A} \in \mathbb{R}^{I \times F}$,$\mathit{B} \in \mathbb{R}^{J \times F},\mathit{C} \in \mathbb{R}^{K \times F}$ from an independent normal distribution to generate the huge tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$ where we set $I=J=K$ ranging from 1000 to 10000 and the rank F is set to be a constant small value 5. On the compression stage, we set the size of compressed tensor cubes $\mathcal{Y}_{p} \in \mathbb{R}^{L \times M \times N}$ as same value $L=M=N=50$. The size of one tensor block $\mathit{B} \in \mathbb{R}^{d_{1} \times d_{2} \times d_{3}}$ on the compression stage is set as $d_{1}=d_{2}=d_{3}=500$ while it is set as $d_{1}=20,d_{2}=40$ and $d_{3}=60$ on the scaling and permutation stage.  We set P as $\max(\frac{I-2}{L-2},\frac{J}{M},\frac{K}{N})$+10 to avoid the situation that  if the CP tensor decomposition of one or a little more  compression  replicas can't converge on the factorization stage,  drop it (them) in time. 

For the evaluation of factorization for sparse tensos, we test cases on scales ranging from one to six  hundred million. The generation of large scale tensors $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$ is similar with that for dense tensors but set the number of non-zero elements in each mode matrix as one hundredth  of the dimension. We denote the  size of compression replica $\mathcal{Y} \in \mathbb{R}^{L \times M \times N}$ as $L=\frac{I}{10},M=\frac{J}{10},N=\frac{K}{10}$. 

For the evaluation of exascale tensors, we test case for exascale tensor with ranging the sparsity. For each cases, we ranges the number of non-zero elements of the mode matrices to control the sparsity of the exascale tensors. 


\subsection{Experimental Results}
\subsubsection{Sparse Tensor Decomposition}
\begin{figure}[t]
    \centering
    \includegraphics[width=3in]{Figures/sparseTime.png}
    \caption{Comparison of time performance between baseline and optimized version.}
    \label{sparsetime}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=3in]{Figures/sparseError.png}
    \caption{Comparison of reconstruction mean squared error (MSE) between baseline and optimized version.}
    \label{sparseerror}
\end{figure}

Figure \ref{sparsetime} shows the comparison of time performance between the baseline and the optimized versions. Compared to the baseline,   the optimized version on GPUs achieves an average of $17.17 \times$ speedups with up to $34.60 \times$ speedups. For tensor of size $6,000 \times 6,000 \times 6,000$, we reduce the baseline time of three and a half hours to nearly 6 minutes.

Figure \ref{sparseerror} shows the comparison of MSE between the baseline and the optimized version. It can be seen that the all the MSE are increasing as the scale increases,  but all of them control the error under the magnitude of $10^{-15}$.  

Using only one compression replica and compressive sensing method makes the decomposition of sparse tensors heavily restricted by the   factorization stage for the limited VRAM. In our experiment, the max size of tensor that can handle on GPU is $6,000 \times 6000 \times 6000$ when the compression rate is denoted as $10$ on the compression stage.


\subsubsection{Dense Tensor Decomposition}
\begin{figure}[t]
    \centering
    \includegraphics[width=3in]{Figures/newTime.png}
    \caption{Comparison of time performance between baseline and optimized version.}
    \label{densetime}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=3in]{Figures/newCost.png}
    \caption{Comparison of reconstruction mean squared error(MSE) between baseline and optimized version.}
    \label{denseerror}
\end{figure}

Figure \ref{densetime} shows the comparison of time performance between the baseline and the optimized version. Compared to the baseline,  the optimized version on CPUs achieves an average of $2.18 \times$ speedups  with up to $2.77 \times$ speedups, and the optimized version on GPUs achieves an average of $4.92 \times$ speedups with up to $6.95 \times$ speedups. For trillion-scale tensor of size $10,000 \times 10,000 \times 10,000$, we reduce the baseline time of nearly half a day to no more than 6 hours.

Figure \ref{denseerror} shows the comparison of MSE between the baseline and the optimized versions. It can be seen that the all the MSE are increasing as the scale increases,  but all of them control the error under the magnitude of $10^{-7}$. Comparing to the baseline, the parallel scheme on CPUs is almost the same with more than $2 \times$ speedups. For the parallel scheme on GPUs, it trades just a little more loss for the significant acceleration. 

\subsubsection{Exascale-Tensor Decomposition}
\begin{figure}[t]
    \centering
    \includegraphics[width=3in]{Figures/TwoStageTime.png}
    \caption{Comparison of time performance between baseline and optimized version.}
    \label{twostagetime}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=3in]{Figures/TwoStageError.png}
    \caption{Comparison of reconstruction mean squared error(MSE) between baseline and optimized version.}
    \label{twostageerror}
\end{figure}

Figure \ref{twostagetime} shows the comparison of time performance between the baseline and the optimized version. Compared to the baseline,  the optimized version on GPUs achieves an average of $56.52 \times$ speedups with up to $172.98 \times$ speedups. For trillion-scale tensor of size $10,000 \times 10,000 \times 10,000$, we reduce the baseline time of nearly half $18$ hours to merely $20$ minutes.

Figure \ref{twostageerror} shows the comparison of MSE between the baseline and the optimized version. It can be seen that the all the MSE are increasing as the scale increases,  but all of them control the error under the magnitude of $10^{-14}$. 

Compared with directly using compressive sensing method with only one replica or factorization large scale tensors with no assumption of sparsity, \textit{Exascale-Tensor} can factorize large scale tensors with more efficiency and less lost for precision. 




==> dac24/Sections/The_Proposed_Solution.tex <==
\section{Exascale CP Tensor Decomposition}
\label{SEC_IMPLEMENTATION}

\begin{algorithm}[t] 
\caption{Exascale-Tensor Scheme} 
\label{alg:Twice compression Framwork} 
\begin{algorithmic}[1] %这个1 表示每一行都显示数字
\REQUIRE ~~\\ %算法的输入参数：Input
sparse tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$ with rank F; dimensions of first compression replicas, $L, M, N$;dimensions of second compression replicas, $qL, qM, qN$; the number of replicas $P$; the number of common columns $S$.
\ENSURE %算法的输出：Output
matrices $(\bm{A}, \bm{B}, \bm{C})$.\\
\STATE Randomly generate matrices $\bm{U}_{p} \in \mathbb{R}^{qL \times L},\bm{V}_{p} \in \mathbb{R}^{qM \times M},\bm{W}_{p} \in \mathbb{R}^{qN \times N}$, $p=1,2, .., P$, and set the first $S$ columns the same, and randomly generate matrices $\bm{U} \in \mathbb{R}^{L \times I},\bm{V} \in \mathbb{R}^{M \times J},\bm{W} \in \mathbb{R}^{N \times K}$,


\STATE $\mathcal{Y}_{p} \gets$ compress $\mathcal{X}$ using $(\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{V},\bm{W}_{p}\bm{W})$ according to  Eq. (\ref{compression_equation}), for $p = 1, .., P$,
%\ENDFOR
\label{code:fram:factorization}
\FOR{$p=1$ to $P$} 
\STATE $(\bm{A}_{p}, \bm{B}_{p}, \bm{C}_{p})$ $\gets$ rank-R CP decomposition  of $\mathcal{Y}_{p}$ via Alg. \ref{alg:baseline CP},
\STATE $(\bm{A}_{p},\bm{B}_{p},\bm{C}_{p})\gets$  divide each column of $(\bm{A}_{p},\bm{B}_{p},\bm{C}_{p})$ by the maximum of the first $S$ rows, respectively,
%\STATE $\Bar{\bm{A}_{p}}$ $\gets$ the first S rows of $\bm{A}_{p}$,
\STATE $\bm{\Pi}_{p}$ $\gets$  $\argmax_{\bm{\Pi}} \text{Tr}(\bm{A}_{1}(1:S, :)^{T}\bm{A}_{p}(1:S, :)\bm{\Pi})$,
\STATE $(\bm{A}_{p},\bm{B}_{p},\bm{C}_{p}) \gets$  $(\bm{A}_{p}\bm{\Pi}, \bm{B}_{p}\bm{\Pi}, \bm{C}_{p}\bm{\Pi})$,
\ENDFOR
\label{code:fram:join}
\STATE $(\bm{A}^{*}, \bm{B}^{*}, \bm{C}^{*})$ $\gets$ solve  the least squares problem (\ref{lsq}) per mode,
\STATE $(\hat{\bm{A}},\hat{\bm{B}},\hat{\bm{C}})$ $\gets$ rank-R CP decomposition of $\mathcal{B}_{1}$,
\STATE $\bm{\Pi},\bm{\Sigma}$ $\gets$ match $\hat{\bm{A}}$ with the first $d_{1}$ rows of $\bm{A}^{*}$ using the Hungarian algorithm.
\STATE $\bm{A}^{'}$ $\gets$ $\bm{A}^{*}\bm{\Pi}\bm{\Sigma}$,
\STATE Repeat line 11-12 for $\bm{B}^{'}$ and $\bm{C}^{'}$, respectively,
\STATE $\bm{A} \gets $ use OMP algorithm to solve for the $L_{1}$ constraint minimization problem $\bm{A}^{'} = \bm{U}\bm{A}$, and likewise for $\bm{B}$ and $\bm{C}$,
\label{code:fram:join}

\RETURN $(\bm{A}, \bm{B}, \bm{C})$.
\end{algorithmic}
\end{algorithm}


In this section, we first briefly introduce the flow of our \textit{Exascale-Tensor} scheme, and then describe its four stages: compression, factorization, recovering the permutation and scaling, and compression sensing stages.  

\subsection{Overview}

% 用词需要统一  名词  动词 需要一致 
\begin{figure*}[t]
    \centering
    \includegraphics[height = 5cm, width = 18cm]{Figures/modify.jpg}
    \caption{Overview of the proposed \textit{Exascale-Tensor} decomposition, where the tensor $\mathcal{X} \in \mathbb{R}^{300 \times 300 \times 300}$, the amount P of the compression replicas $\mathcal{Y}$ is 8 $\ge \max(\frac{300-2}{50-2},\frac{300}{50},\frac{300}{50})$.}
    \label{pic_one-parallelization-schemes}
\end{figure*}



The \textit{Exascale-Tensor} algorithm mainly consists of of four stages, namely compression stage, factorization stage, recovering permutation and scaling stage, and compression sensing stage as shown in Fig. \ref{pic_one-parallelization-schemes}. The pseudo code  for \textit{Exascale-Tensor} is shown in Alg. \ref{alg:Twice compression Framwork}.


% 对应着图上的阶段名字
% 先讲图，再讲算法，算法第几行到第几行对应哪部分....

%First, a tensor $\mathcal{X} \in \mathbb{R}^{300 \times 300 \times 300}$, consisting of $27$ tensor blocks $\mathcal{B}_{n} \in \mathbb{R}^{100 \times 100 \times 100}$, $n=1, 2, ..., 27$, is first compressed into $8$ replicas $\mathcal{Y}_{p} \in \mathbb{R}^{50 \times 50 \times 50}$, $p=1, 2, ..., 8$. Second, using CP decomposition, each replica is factored to matrices independently. Thirdly, with a proper permutation and normalization, solving a least squares problem for each mode will result in the factorization matrices $(\bm{A}^{*},\bm{B}^{*},\bm{C}^{*})$. Using the factorization of the first block $\mathcal{B}_{1}$, we get the permutation matrix $\bm{\Pi}$ and the scaling matrix $\bm{\Sigma}$. Then, we use $\bm{\Pi}$ and $\bm{\Sigma}$ to obtain the full mode matrices $(\bm{A},\bm{B},\bm{C})$. 

%First, a tensor $\mathcal{X} \in \mathbb{R}^{200 \times 200 \times 200}$ of rank $5$, is divided into $8$ blocks $\mathcal{B}_{n} \in \mathbb{R}^{100 \times 100 \times 100}$, $n=1, 2, ..., 8$, and then  compressed into $3$ replicas $\mathcal{Y}_{p} \in \mathbb{R}^{50 \times 50 \times 50}$, $p=1, 2, 3$, where the $n$-th block $\mathcal{B}_{n}$ is compressed into $\mathcal{Y}_{p}^{n}$ by $\bm{U}_{p},\bm{V}_{p}$  and $\bm{W}_{p}$ which are the generated random compression matrices introduced in Section \ref{compression_based_demo}, and $\mathcal{Y}_{p}=\sum\limits_{n}\mathcal{Y}_{p}^{n}$, $p=1, 2, 3$, $n=1, 2, ..., 8$.

First,  a sparse tensor $\mathcal{X} \in \mathbb{R}^{300 \times 300 \times 300}$ of rank $5$, is divided into $27$ blocks $\mathcal{B}_{n} \in \mathbb{R}^{100 \times 100 \times 100}$, $n=1, 2, ..., 27$. Each block $\mathcal{B}_{n}$ will be compressed $8$ times by $\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{V}$ and $\bm{W}_{p}\bm{W}$, where $\bm{U}_{p}, \bm{V}_{p},\bm{W}_{p} \in \mathbb{R}^{50 \times 80}$, $p=1, 2, .., 8$, and  $\bm{U}, \bm{V}, \bm{W} \in \mathbb{R}^{80 \times 100}$, which are the generated random compression matrices introduced in Section \ref{compression_based_demo}.   Specifically, the $n$-th block $\mathcal{B}_{n}$ is compressed into $\mathcal{Y}_{p}^{n}$, $p=1,2,..., 8$. Then, by 
adding all the $p$-th replicas of each block,  we can get the $p$-th replica of the original tensor $\mathcal{X}$,  $\mathcal{Y}_{p}$.  That is,  $\mathcal{Y}_{p}=\sum\limits_{n}\mathcal{Y}_{p}^{n}$,   $p=1, 2,..., 8$,  $n=1, 2, ..., 27$,  $\mathcal{Y}_{p} \in \mathbb{R}^{50 \times 50 \times 50}$.

Second, using CP decomposition, each replica $\mathcal{Y}_{p}$ is factored to matrices, $\bm{A}_{p} \in \mathbb{R}^{50 \times 5}$, $\bm{B}_{p} \in \mathbb{R}^{50 \times 5}$,  $\bm{C}_{p} \in \mathbb{R}^{50 \times 5}$, $p=1, 2,..., 8$. Note that the compression of $\mathcal{X}$ by $\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{V}$ and $\bm{W}_{p}\bm{W}$, can be written as
\begin{equation}
\begin{split}
    \bm{y}_{p}&=\text{Vec}(\bm{Y}_{p})\\
    &=(({(\bm{U}_{p}\bm{U})}\otimes{(\bm{V}_{p}\bm{V})}\otimes{(\bm{W}_{p}\bm{W})})(\bm{A}\odot\bm{B}\odot\bm{C}))\bm{1}\\
    &=((\bm{U}_{p}\bm{U}\bm{A})\odot(\bm{V}_{p}\bm{V}\bm{B})\odot(\bm{W}_{p}\bm{W}\bm{C}))\bm{1},
\end{split}
\end{equation}
 where $\bm{A}, \bm{B}$ and $\bm{C}$ are the factorization matrices of $\mathcal{X}$. According to the definition of CP decomposition, the factorization of the replica $\mathcal{Y}_{p}$ can be written as 
 \begin{equation}
 \begin{split}
 \bm{y}_{p}=(\bm{A}_{p}\odot\bm{B}_{p}\odot\bm{C}_{p})\bm{1}
 \end{split}
 \end{equation}
 Therefore, due to the uniqueness of CP decomposition up to scaling and permutations, we have 
 \begin{equation}
 \begin{split}
 \bm{A}_{p}&=\bm{U}_{p}\bm{U}\bm{A}=\bm{U}_{p}\bm{U}\bm{A}\bm{\Pi}_{p}\bm{\Sigma}_{p}^{a},\\
 \bm{B}_{p}&=\bm{V}_{p}\bm{V}\bm{B}=\bm{V}_{p}\bm{V}\bm{B}\bm{\Pi}_{p}\bm{\Sigma}_{p}^{b},\\
 \bm{C}_{p}&=\bm{W}_{p}\bm{W}\bm{C}=\bm{W}_{p}\bm{W}\bm{C}\bm{\Pi}_{p}\bm{\Sigma}_{p}^{c}
 \end{split}
 \end{equation}
 where $\bm{A}, \bm{B}, \bm{C}$ are the CP factorization matrices of $\mathcal{X}$ as shown in Eq. (\ref{cp_equation}), $\bm{\Pi}_{p}$ is the column permutation matrix, $\bm{\Sigma}_{p}$ is the column scaling matrix and $\bm{\Sigma}_{p}^{a}\bm{\Sigma}_{p}^{b}\bm{\Sigma}_{p}^{c}=\bm{I}$. Using Hungarian algorithm and dividing by the maximum elem in each column, the factored matrices have a common permutation and scaling which satisfy 
 \begin{equation}
 \begin{split}
 \bm{A}_{p}&=\bm{U}_{p}\bm{U}\bm{A}\bm{\Pi}\bm{\Sigma}^{a},\\  \bm{B}_{p}&=\bm{V}_{p}\bm{V}\bm{B}\bm{\Pi}\bm{\Sigma}^{b},\\ \bm{C}_{p}&=\bm{W}_{p}\bm{W}\bm{C}\bm{\Pi}\bm{\Sigma}^{c}. 
 \end{split}
 \end{equation}
 Then, using a least square method for each mode will result in the factorization matrix $\bm{A}^{*},\bm{B}^{*}$ and $\bm{C}^{*}$ which satisfy
 \begin{equation}
\begin{split}
 \bm{A}^{*}&=\bm{U}\bm{A}\bm{\Pi}\bm{\Sigma}^{a}, \\ \bm{B}^{*}&=\bm{V}\bm{B}\bm{\Pi}\bm{\Sigma}^{b},\\  \bm{C}^{*}&=\bm{W}\bm{C}\bm{\Pi}\bm{\Sigma}^{c}.
\end{split}
\end{equation}
Third, because of the uniqueness of CP decomposition, using the factorization of a compression replica for the first block $\mathcal{B}_{1}$ using $\{\bm{U}, \bm{V}, \bm{W}\}$, we can get the permutation matrix $\bm{\Pi}$ and the scaling matrices $\bm{\Sigma}^{a}$, $\bm{\Sigma}^{b}$ and $\bm{\Sigma}^{c}$. We use  the permutation and scaling matrices  to obtain $(\bm{A'},\bm{B'},\bm{C'})$, where we have
\begin{equation}
\label{last equation}
\begin{split}
\bm{A'}&=\bm{U}\bm{A}\\
\bm{B'}&=\bm{V}\bm{B}\\
\bm{C'}&=\bm{W}\bm{C}    
\end{split}
\end{equation}
Last, exploiting the sparsity of $\mathcal{X}$, we use OMP algorithm to solve the $L_{1}$ constraint minimization problems as shown in Eq. (\ref{last equation}), and obtain the full mode matrices $\bm{A}$, $\bm{B}$ and $\bm{C}$. 


%Thirdly, after a proper permutation and scaling for columns  of factored matrices, solving a least squares problem for each mode will result in the factorization matrices  $(\bm{A}^{*},\bm{B}^{*},\bm{C}^{*})$. Using the factorization of the first block $\mathcal{B}_{1}$, we get the permutation matrix $\bm{\Pi}$ and the scaling matrix $\bm{\Sigma}$. Then, we use $\bm{\Pi}$ and $\bm{\Sigma}$ to obtain the full mode matrices $(\bm{A},\bm{B},\bm{C})$.



%For the sparse tensors, the $\textit{trillion-tensor}$ algorithm mainly consists of two stages, namely the compression stage same as that in the $\textit{trillion-tensor}$ algorithm for dense tensors but here only one replica being created, and factorization stage composed of tensor decomposition in compressed domain and recovery of mode matrices in uncompressed space as given in Alg. \ref{alg:Framworkforsparse}. It differs from the algorithm for dense tensors mainly in the factorization stage which it utilizes the compressed sensing theory to directly solve the sparsity-constrained linear system per-mode for restoring the mode matrices in uncompressed space. 








% 点名计算任务

\subsection{Compression Stage}

The compression stage is corresponding to line 1--2  in  Alg. \ref{alg:Twice compression Framwork}. To compress tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$ into $\mathcal{Y} \in \mathbb{R}^{L \times M \times N}$, the $(i,j,k)$-th element of $\mathcal{Y}$ is computed as follows: 
\begin{equation}
\label{compression_equation}
    \mathcal{Y}_{lmn}=\sum\limits_{i=1}^{I}\sum\limits_{j=1}^{J}\sum\limits_{k=1}^{K}\bm{U}_{li}\bm{V}_{mj}\bm{W}_{nk}\mathcal{X}_{ijk},
\end{equation}
where $\bm{U}\in\mathbb{R}^{L \times I} , \bm{V}\in\mathbb{R}^{M \times J}, \bm{W}\in\mathbb{R}^{N \times K}$ are random matrices from the normal distribution. %It can be seen as an iterative steps: reshape $\bm{U}^{T}\bm{X}_{(1)}$ to $\mathcal{G} \in \mathbb{R}^{L \times J \times K}$, then reshape $\bm{W}^{T}\bm{G}_{(3)}$  to $\mathcal{G} \in \mathbb{R}^{L \times J \times N}$, and finally reshape $\bm{V}^{T}\bm{G}_{(2)}$ to $\mathcal{Y}$ as we wanted.

In \textit{Exascale-Tensor}, $\mathcal{X}$ will be compressed twice. \mathcal{X} is first compressed into one relative small replica $\mathcal{Y} \in \mathbb{R}^{L \times M \times N}$. Then $\mathcal{Y}_{p}$ will be compressed  into P replicas $\mathcal{Y}_{p} \in \mathbb{R}^{qL \times qM \times qN}$, $p=1,2,...,P$,  $P \ge \max(\frac{L-2}{qL-2},\frac{M}{qM},\frac{N}{qN})$. Two continuous compression can be  equivalent to  one time of compression for $\mathcal{X}$ using $(\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{V},\bm{W}_{p}\bm{W})$.



%While for the sparse tensors, there is only one replica needed, i.e., $P=1$, but the compression rate will be constrained due to the compressed sensing theory, $I \gg L > 2K_{A}$, where $K_{A}$ is the latent sparsity of the load matrix $\bm{A}$ along the I-mode of the tensor, and likewise for the J-mode and K-mode. 




To process an ``out-of-memory" tensor, we adopt a spliting  strategy that we first split $\mathcal{X}$ into multiple blocks $\mathcal{B}_{n} \in \mathbb{R}^{d_{1} \times d_{2} \times d_{3}}$ $n=1,2,...,\frac{IJK}{d_{1}d_{2}d_{3}}$ as shown for example in Fig.  \ref{pic_one-parallelization-schemes}. Then, due to the block tensor operation, we exploit the related components of $(\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{U},\bm{W}_{p}\bm{W})$ to compress each block $\mathcal{B}_{n}$ to replicas $\mathcal{Y}_{p}^{n}$, $p=1,2,...P$, where $\bm{U}_{p} \in \mathbb{R}^{qL \times L}$, $\bm{V}_{p} \in \mathbb{R}^{qM \times M}$, $\bm{W}_{p} \in 
\mathbb{W}_{p} \in \mathbb{R}^{qN \times N}$ and $\bm{U} \in \mathbb{R}^{L \tiems I}$, $\bm{V} \in \mathbb{R}^{M \times J}$,  $\bm{W} \in \mathbb{R}^{N \times K}$, $P \ge \max(\frac{L-2}{qL-2},\frac{M}{qM},\frac{N}{qN})$, $L \ge 2K_{A}$, $M \ge 2K_{B}$ $N \ge 2K_{C}$, $\{K_{A},K_{B},K_{C}\}$ denoted as the latent sparsity of $\mathcal{X}$ along each mode respectively. Finally,  accumulate them to the final replicas $\mathcal{Y}_{p}$ respectively, i.e.,  $\mathcal{Y}_{p}+=\mathcal{Y}_{p}^{n}$,   $p=1,2,..,P$.
% Different from directly using $\{\bm{U}_{p},\bm{V}_{p},\bm{W}_{p}\}$ in \textit{Trillion-Tensor}, we use   $\{\bm{U}_{p}\bm{U},\bm{V}_{p}\bm{V},\bm{W}_{p}\bm{W}\}$ to compress the large tensor. The  use of additional matrix further improve the compression ratio and exploiting the latent sparsity of $\mathcal{X}$ for following compression sensing stage.



%The essential of the compression stage is to multiply every slab of the tensor $\mathcal{X}$ from the I-mode with $\bm{U}_{p}^{T}$, the J-mode with $\bm{V}_{p}^{T}$ and the K-mode with $\bm{W}_{p}^{T}$. To address the terrible situation that we can not load the full large tensor $\mathcal{X}$ into RAM, we adopt the strategy that we first split the large tensor into some  tensor blocks $\mathcal{B}_{n} \in \mathbb{R}^{d_{1} \times d_{2} \times d_{3}}$ with the number of $\frac{I \times J \times K}{d_{1} \times d_{2} \times d_{3}}$ as shown for example in Figure \ref{pic_one-parallelization-schemes}, then multiply each tensor block $\mathcal{B}_{n}$ read in RAM with corresponding mode compression sub-matrices  to get one component of the replica $\mathcal{Y}_{p}^{\mathcal{B}_{n}}$, and finally accumulate it to the final replica $\mathcal{Y}_{p}$.
   

\subsection{Factorization Stage}

The factorization stage is  involved in line 3--9 of Alg. \ref{alg:Twice compression Framwork}. On the factorization stage, each replica $\mathcal{Y}_{p}$ will be independently factored to $(\bm{A}_{p},\bm{B}_{p},\bm{C}_{p})$, $p=1,2,..,P$, using the CP decomposition shown in Alg.\ref{alg:baseline CP}. Due to a property of the Kronecker product \cite{kr_property}, we have the equation $\bm{A}_{p}=\bm{U}_{p}\bm{U}\bm{A}\bm{\Pi}_{p}\bm{\Sigma}_{p}$,  $p=1,2,...,P$.  Here, we apply Hungarian algorithm \cite{HA} to  the trace maximization problem to get rid of $\bm{\Pi}_{p}$ and divide each column by  its maximum of the first S rows to get rid of $\bm{\Sigma}_{p}$, where we $S$ is the number of shared columns in the random matrices $\bm{U}_{p}, p=1,2,...,P$. Finally, solve a master least squares problem 
\begin{equation}
\label{lsq}
\left[
\begin{array}{c}
     \bm{A}_{1}\\
     \vdots    \\
     \bm{A}_{P}\\
\end{array}
\right]
=
\left[
\begin{array}{c}
    \bm{U}_{1} \\ 
    \vdots    \\
    \bm{U}_{P}
\end{array}
\right]
\bm{U}\bm{A}\bm{\Pi}\bm{\Sigma}
\end{equation}
to obtain $\bm{A}^{*} =\bm{U}\bm{A}\bm{\Pi}\bm{\Sigma}$,  and similarly for $\bm{B}^{*}$ and $\bm{C}^{*}$.

%For sparse tensors, on the factorization stage, the replica $\mathcal{Y}$ will be first factored to $(\bm{A}_{y},\bm{B}_{y},\bm{C}_{y})$. Due to a property of the Kronecker product, we have the constraint $\bm{A}_{y}=\bm{U}^{T}\bm{A}$. Different from the solution for dense tensors, the load matrix $\bm{A} \in \mathbb{R}{I \times F}$ is sufficiently sparse with supposed sparsity  $K_{A}$, with the projection matrix $\bm{U} \in \mathbb{R}^{L \times I}$ which satisfies $I \gg L > 2K_{A}$. Thus, this problem can be rewritten as an classical $l_{0}$ constraint minimization problem
%\begin{equation}
%\label{compression_equation_for_sparse}
%    \min\limits_{A}{\Vert\bm{A}_{y}-\bm{U}\bm{A}\Vert}_{%2}^{2} \textit{ subject to }  {\Vert\bm{A}\Vert}_{0} %\leq K_{A},
%\end{equation}

%where ${\Vert\bm{A}\Vert}_{0}$ is the $L_{0}$ pseudo-norm, i.e. the number of nonzero elements in $\bm{A}$.  According to the compressed sensing theory, it is natural to regard $\bm{A}$ as the latent sparse signals in high-dimension uncompressed space, $\bm{U}$ as the dictionary, and $\bm{A}_{y}$ as the observation signals in low-dimension compression domain. Here, we exploit  OMP-Cholesky  algorithm to solve the sparse-constraint least square problem to obtain $\bm{A}$ and likewise for $\bm{B}$ and $\bm{C}$.  

\subsection{Recovering Scaling and Permutations}

The recovering scaling and permutation stage is involved in line 10--13 of Alg. \ref{alg:Twice compression Framwork}. To recover the scaling and permutations, we use the factors $(\hat{\bm{A}},\hat{\bm{B}},\hat{\bm{C}})$ of the compression replica for first block $\mathcal{B}_{1}$ using $\{\bm{U},\bm{V},\bm{W}\}$ as compression matrices. Because the CP tensor decomposition is unique, we assume that $(\hat{\bm{A}},\hat{\bm{B}},\hat{\bm{C}})$ are the first $d_{1}$ rows of full mode matrices $(\bm{A}^{*},\bm{B}^{*},\bm{C}^{*})$, i.e., $\hat{\bm{A}}={\bm{A}^{*}}(1:d_{1},:)\bm{\Pi}\bm{\Sigma}$. Here, we make the diagonal entries of the scaling  matrix $\bm{\Sigma}$ composed of  the maximums of each column in $\hat{\bm{A}}$, i.e. $\bm{\bm{\Sigma}}=\text{diag}( \max(\hat{\bm{A}}(:,1)), ..., \max(\hat{\bm{A}}(:,F) ) )$. To obtain  the full mode matrix $\bm{A}^{'}$  for the compression replica of $\mathcal{X}$ using $(\bm{U},\bm{V},\bm{W}$), first, we divide each column of $\hat{\bm{A}}$ by its maximum and divide each column of $\bm{A}^{*}$ by its maximum of the first $d_{1}$ rows.  Second,  similar to the factorization stage, we apply the Hungarian algorithm \cite{HA} to maximize $\text{Tr}({\hat{\bm{A}}}^{T}{\bm{A}^{*}}(1:d_{1},:)\bm{\Pi})$ and obtain the permutation matrix $\bm{\Pi}$. Thus, we get the mode matrix $\bm{A}^{'}=\bm{U}\bm{A}^{*}\bm{\Pi}\bm{\Sigma}$, similarly for $\bm{B}^{'}$ and $\bm{C}^{'}$.




%/In practice, we usually make the first block on this stage,  $\mathcal{B}_{1} \in \mathbb{R}^{d_{1} \times d_{2} \times d_{3}}$, to be different from that on the compression stage in the size. And in our experiment of the large-scale tensor decomposition, it is proved to be effective if we  set $d_{1} \neq d_{2} \neq d_{3}$ and make the size of the tensor block on current stage smaller than that on the compression stage when the rank $F$ of tensor $\mathcal{X}$ is relative smaller than the size of tensor. 




\subsection{Compression Sensing Stage}

The compression sensing stage corresponds to line 14 of Alg. \ref{alg:Twice compression Framwork}. 
Compression sensing can be formally described as 
\begin{equation}
    \bm{Y}=\bm{U}\bm{A},
\end{equation}
where $\bm{Y} \in \mathbb{R}^{L \times F}$ denoted as measurement matrix, $\bm{U} \in \mathbb{R}^{L \times I}$ denoted as the dictionary, $\bm{A} \in \mathbb{R}^{I \times F}$ denoted as the sparse   signal matrix. 

For $\bm{A'},\bm{B'}$ and $\bm{C'}$ obtained on the recovering stage and  we have $\bm{A'}=\bm{U}\bm{A}$, $\bm{B'}=\bm{V}\bm{B}$ and $\bm{C'}=\bm{W}\bm{C}$ where $\bm{A},\bm{B}$ and $\bm{C}$ are sparse. So, it is equivalent to the the compression sensing problem and  we can use $L_{1}$ constraint minimization algorithm OMP to solve the problems to obtain full mode matrices $\bm{A}$, $\bm{B}$ and $\bm{C}$.






%On the compression stage, the \textit{Exascale-Tensor} scheme reads block tensor from memory, alternatively utilize the tensor matricization and matrix multiplication in each axis to compress large tensor to small replicas. This process consists of data-independent operations including matrix transport, tensor matricization and matrix multiplication which are suitable for parallel computations.  

%Besides, the compression of all replicas and the decomposition of each replica is also independent with each other which is suitable for parallel computations.

%Thus, we propose to offload the data-independent and high parallel computations from CPU to GPU which is of effect for massive parallel computations.   We furthermore performed preliminary experiments to evaluate the GPU implementation of \texit{Trillion-Tensor}  and observed that low memory access efficiency, expensive device communication and low utilization of GPUs are the bottlenecks restricting the performance of our scheme. Therefore, we mainly focus on optimization these aspects in the following context. 




%The last stage is designed for mode estimation matrices $(\bm{A}^{*},\bm{B}^{*},\bm{C}^{*})$ to recover  the scaling and permutations.
%Resort to the uniqueness of CP tensor decomposition and the property of low rank for tensors, intuitively, for a given large tensor $\mathcal{X} \in \mathbb{R}^{I \times J \times K}$, we might as well assume the factorization mode matrices $(\bm{A}',\bm{B}',\bm{C}')$ of the sub tensor block $\mathcal{B}_{1}$, located in the first corner as shown for example in Figure \ref{pic_one-parallelization-schemes},  is same with the corresponding sub-matrices of the factorization mode matrices $(\bm{A},\bm{B},\bm{C})$ from the full tensor. 

%From this point of view, to recover from the permutations and scaling for mode estimation matrices we get on the factorization stage, we can make full use of the factorization result $(\bm{A}',\bm{B}',\bm{C}')$ of the tensor block $\mathcal{B}_{1}$. Due to the uniqueness of CP tensor decomposition and the property of low rank for tensors, we have the constraint equation $\bm{A}^{*}'= \bm{A}'\bm{\Pi}\bm{\Sigma}$ (likewise for $\bm{B}^{*}$ and $\bm{C}^{*}$), where $\bm{A}^{*}'$ is the corresponding sub-matrix of $\bm{A}^{*}$ related to $\bm{A}'$, and $\bm{\Pi}$, $\bm{\Sigma}$ are the permutation and scaling matrices. Similarly to the factorization stage, to get ride of the permutation matrix $\bm{\Pi}$, we apply the Hungarian algorithm for matching the normalized mode estimation sub matrix $\bm{A}^{*}'$ with the normalized $\bm{A}'$. After permutation, we multiply corresponding column factors of anchor mode matrices to normalized estimation matrices to get rid of the scaling matrix $\bm{\Sigma}$.

 




%\subsection{Optimizations}
%The computational complexity of the compression stage is $O(PIJK \times \min(L,M,N))$ versus $O(\frac{IJ}{F})$ of the factorization stage \cite{paracomp}.  Huge time consumption of the compression stage is the bottleneck of this algorithm with the size of tensor increasing.  

%On the compression stage, operations of all tensor blocks $\mathcal{B}_{n}, n=1, 2, ..., \frac{IJK}{d_{1}d_{2}d_{3}}$, are independent of each other, and the respective compression result $\mathcal{Y}_{p}^{n}$  will be accumulated to the  common replica $\mathcal{Y}_{p}$, $p=1,2,..., P$. There is $\frac{IJK}{d_{1}d_{2}d_{3}}$ parallelism in this process. Thus, we design two parallelization schemes for efficient compression on CPUs and GPUs, respectively. 


%\textbf{Parallel implementation on CPUs}: This scheme advocates exploiting the property of multi-core processors on CPUs. In this scheme, we compress the tensor block $\mathcal{B}_{n}$, $n=1,2,...,\frac{IJK}{d_{1}d_{2}d_{3}}$, in parallel on multi processes. On each sub-process, one of tensor blocks, $\mathcal{B}_{n}$, will be loaded in memory and  independently compressed into sub-replicas $\mathcal{Y}_{p}^{n}$, $p=1,2,...,P$, then the sub-replicas will be accumulated to corresponding common  replicas $\mathcal{Y}_{p}$ shared on the main process,  $p=1,2,...,P$.

%\textbf{Parallel implementation on GPUs}: 
%This scheme advocates exploiting GPUs' high performance in matrix multiplication. Consider a given situation that for a trillion-scale tensor $\mathcal{X} \in \mathbb{R}^{10,000 \times 10,000 \times 10,000}$ composed of tensor blocks $\mathcal{B}_{n} \in \mathbb{R}^{500 \times 500 \times 500}$, $n=1,2,...,8000$, there are    $3 \times 8,000$ times of matrix multiplication need to be done. The huge time consumption of extra large-scale matrix multiplication on CPUs is always unbearable. However, compared to CPU, GPU is more suitable for large-scale matrix multiplication for its much greater number of relatively unexceptional processing cores.

%Thus, compared to the parallel implementation on CPUs, this scheme differs only in the matrix computation step, in which it transfer the block $\mathcal{B}_{n}$ of each sub-process from CPUs to GPUs and the following compression steps except the accumulation will work on GPUs. The accumulation step will first transfer $\mathcal{Y}_{p}^{n}$, $p=1,2,...,P$ to CPUs and then accumulate them to corresponding replicas.


%Because of the parallelism of the multiplication of tensor blocks with related random mode sub-matrices $\bm{U}_{p}^{'}, \bm{V}_{p}^{'},\bm{W}_{p}^{'}$, in our work, we put the the compression of the tensor block $\mathcal{B}_{n}$ on multi processes, and set the replica set ${\{\mathcal{Y}_{p}\}}_{p=1,2,...,P}$ on the main process to be shared with sub-processes, i.e., on each process, we independently compress one tensor block $\mathcal{B}_{n}$ to a series of sub-replicas ${\{\mathcal{Y}_{p}^{\mathcal{B}_{n}}\}}_{p=1,2,...,P}$, and corresponding accumulate them to replicas set ${\{\mathcal{Y}_{p}\}}_{p=1,2,...,P}$ on the main process.


%Consider a given situation that for a trillion-scale tensor $\mathcal{X} \in \mathbb{R}^{1w \times 1w \times 1w}$ composed of tensor blocks $\mathcal{B}_{n} \in \mathbb{R}^{500 \times 500 \times 500}$, there are 8000 blocks need to be compressed and $3 \times 8000$ times of matrix multiplication need to be done. The huge time consumption of extra large-scale matrix multiplication on CPU is always unbearable. However, compared to CPU, GPU is more suitable for large-scale matrix multiplication for its much greater number of relatively unexceptional processing cores. Thus, in order to reduce the huge time consumption of the matrix multiplication, we exploit the characteristic of GPU on matrix multiplication tasks and take the strategy that load the tensor blocks  $\mathcal{B}_{n}$ into the video memory on GPUs in parallel, then compress it to sub-replicas ${\{\mathcal{Y}_{p}^{\mathcal{B}_{n}}\}}_{p=1,2,...,P}$ serially, and finally merge them to  ${\{\mathcal{Y}_{p}\}}_{p=1,2,...,P}$ on the main process. 

%Based on the complexity-order analysis of algorithm,  consider a situation where a big tensor $\mathcalc{X} \in \mathbb{R}^{I \times J \times K}$ and the compression replicas $\mathcalc{Y}_{p} \in \mathbb{R}^{L \times M \times N}$ with number of P, the complexity-order of the compression stage is $O(PIJK\times \min(L,M,N))$ versus $O(\frac{IJ}{F})$ for the factorization stage.  Huge time consuming of the compression stage is the bottleneck of this tensor decomposition algorithm with the size of tensor increasing.

%To reduce the huge time consumption of computation on the compression stage, we exploit the property of multi-cores on CPUs and the powerful matrix computation performance on GPUs,  developing two different acceleration frameworks on CPUs and GPUs respectively to make a preliminary acceleration.
%In our work, we make a preliminary acceleration with a parallel framework embedding in the stage of compressing the tensor block to P compressed tensor cubes, and make full use of high-performance computations for matrix operations on GPU, to as much as possible accelerate the procedure of super huge scale tensor decomposition.



%Specially, In the stage of tensor compression, we carefully design the size of tensor block read in RAM, and put it directly in GPU to be shared with multiple threads. And we directly take out the corresponding mode compression submatrices on GPU for each thread in parallel to reduce the time cost. These tricks reduce the huge time consuming on tensor compression significantly.    




